Evaluation of Noise and Crosstalk in Neutral Atom Quantum Computers

This work explores and evaluates noise and crosstalk in neutral atom quantum computers. Neutral atom quantum computers are a promising platform for analog Hamiltonian simulations, which rely on a sequence of time-dependent Hamiltonians to model the dynamics of a larger system and are particularly useful for problems in optimization, physics, and molecular dynamics. However, the viability of running multiple simulations in a co-located or multi-tenant environment is limited by noise and crosstalk. This work conducts an analysis of how noise faced by simulations changes over time, and investigates the effects of spatial co-location on simulation fidelity. Findings of this work demonstrate that the close proximity of concurrent simulations can increase crosstalk between them. To mitigate this issue, a Moving Target Defense (MTD) strategy is proposed and evaluated. The results confirm that the MTD is a viable technique for enabling safe and reliable co-location of simulations on neutral atom quantum hardware.

==> email_notes.tex <==
Hi all,

I hope this email finds you well! I was reading your paper "Quantum Cloud Computing: A Review, Open Problems, and Future Directions", and came across a line that I had a question about. In the last paragraph of Section 3.1, it is written

    A quantum computer’s resources are typically shared across different users, so additional considerations, such as a job queuing latency or a task compilation latency (Nguyen et al., 2024b), would also need to be considered.



Is there a source that states that the "resources are shared across different users"? Reading the Nguyen et al. paper, it seems it applies more to distributing a workload across multiple QPUs, rather than multi-tenancy of one cloud QPU. Further, it seems specific to the QPUs produced by the company Quantum Brilliance, and not generalized to cloud QPUs.

I'd love some insight on this :) Thank you so much for your time!

Warm regards,
Pranet

https://arxiv.org/abs/2404.11420

==> old_figs_for_reference/fidelity_of_simulation_over_time <==
%PDF-1.4
%öäüß
1 0 obj
<<
/Type /Catalog
/Version /1.4
/Pages 2 0 R
/StructTreeRoot 3 0 R
/MarkInfo 4 0 R
/Lang (en)
/ViewerPreferences 5 0 R
>>
endobj
6 0 obj
<<
/Title (Copy of Your paragraph text)
/Creator (Canva)
/Producer (Canva)
/CreationDate (D:20250711153048+00'00')
/ModDate (D:20250711153048+00'00')
/Keywords (DAGUUZpvS74,BAFue3tXY3U,0)
/Author (Pranet Sharma)
>>
endobj
2 0 obj
<<
/Type /Pages
/Kids [7 0 R]
/Count 1
>>
endobj
3 0 obj
<<
/Type /StructTreeRoot
/K [8 0 R]
/ParentTree 9 0 R
/ParentTreeNextKey 49
>>
endobj
4 0 obj
<<
/Marked true
/Suspects false
>>
endobj
5 0 obj
<<
/Type /ViewerPreferences
/DisplayDocTitle true
>>
endobj
7 0 obj
<<
/Type /Page
/Resources <<
/ProcSet [/PDF /Text /ImageB /ImageC /ImageI]
/ExtGState 10 0 R
/XObject <<
/X8 11 0 R
/X9 12 0 R
/X10 13 0 R
>>
/Font 14 0 R
>>
/MediaBox [0.0 7.920007 1440.0 817.92]
/Contents 15 0 R
/StructParents 0
/Tabs /S
/Parent 2 0 R
/BleedBox [0.0 7.920007 1440.0 817.92]
/TrimBox [0.0 7.920007 1440.0 817.92]
/CropBox [0.0 7.920007 1440.0 817.92]
/Rotate 0
/Annots []
>>
endobj
8 0 obj
<<
/Type /StructElem
/S /Document
/P 3 0 R
/K [16 0 R]
>>
endobj
9 0 obj
<<
/Limits [0 0]
/Nums [0 [17 0 R 18 0 R 19 0 R 20 0 R 21 0 R 22 0 R 23 0 R 24 0 R 25 0 R 26 0 R
27 0 R 28 0 R 29 0 R 30 0 R 31 0 R 32 0 R 33 0 R 34 0 R 35 0 R 36 0 R
37 0 R 38 0 R 39 0 R 40 0 R 41 0 R 42 0 R 43 0 R 44 0 R 45 0 R 46 0 R
47 0 R 48 0 R 49 0 R 50 0 R 51 0 R 52 0 R 53 0 R 54 0 R 55 0 R 56 0 R
57 0 R 58 0 R 59 0 R 60 0 R 61 0 R 62 0 R 63 0 R 64 0 R 65 0 R 18 0 R
20 0 R 22 0 R 23 0 R 24 0 R 26 0 R 27 0 R 29 0 R 30 0 R 32 0 R 34 0 R
35 0 R 36 0 R 38 0 R 39 0 R 41 0 R 42 0 R 44 0 R 46 0 R 47 0 R 48 0 R
50 0 R 51 0 R 53 0 R 54 0 R 56 0 R 57 0 R 58 0 R 60 0 R 62 0 R 63 0 R
65 0 R]
]
>>
endobj
10 0 obj
<<
/G3 66 0 R
/G7 67 0 R
/G11 68 0 R
/G12 69 0 R
/gs5 70 0 R
>>
endobj
11 0 obj
<<
/Length 985
/Type /XObject
/Subtype /Form
/Resources <<
/ProcSet [/PDF /Text /ImageB /ImageC /ImageI]
/ExtGState 71 0 R
>>
/BBox [0 0 7 1425]
/Group 72 0 R
/Filter /FlateDecode
>>
stream
xœE—A®ÜFD÷sŠ¹@~šEªÕ:×ÉÄ{'äþ@0ä#
SßOpSOjýóZïßüˤõèzÿúi½¿¤ç9+ì+ž}¿ÿúùZïϟ?¿½ë‡¿¿~ÿæïïÿ兟/½×ûÇKo½¼V~Fò|C>Ÿ'¹­¼`öù4Õ¥¨KÑ0c×µS×NÃOˆ
tP̪¡ê¡Ý0£ªxUñÕð^]¼ºx4̨.^]ü4Ìÿcu‰êj˜Q]¢ºÄn˜Q]®êr­†Ÿ¸ªËU]®h˜Q]®êr†ŸØÕeW—­†|=|?»aFu¹«Ë½~â®.wu¹£aFu¹«Ë}æ7\]Nu9j˜Q]Nu9»aFuyªË³~â©.Ouy¢aFuyªËsælÖbƒb"^\ß\ßÃ+ÙpØÖðÌr/¹§Ü[î1÷š{ÎìÙ´±hcÒƦQ«6íá•ôcÙækx&ã6ÖmÌÛØ·1pcáægx&#7VnÌÜع1tcé{x%ýX»]kx&ƒ7oLÞؼ1zcõváu[ Ë·­á•ôcý¶÷ðJúa€Ýkx&"&Ø}†g"ƒaƒ¡ƒáƒ!"a"=¼'~XaÏž‰†††††öœáuë䆊Z^ÉM?´öðÊê'ü­á™ø!ü~?"ÂÙž97ü¾ãkx%ýú®ß·ý¾ïã‡ðC}ëÇá‡ðCø!ü~?ägx=^è‡ÂE?"臊=¼'~ø¡k
ÏÄá‡ðCø!ü~è:Ã3ñCø!ü~h÷C³Ÿš{x%ýðC÷ž‰Âá‡ðCø!üÐ}†×#˜~ø!üÐéG4ýðCg¯¤~èYÃ3ñCø!ü~?"zÎpåIaqp'
¯®o®ïá•<ðÃm
ÏÄÇÇÇÇÇ·3<??????\{x%ýúdäkxfŽútÔÇ£>õ©OH}DÂÇÇÇÇÇǏ=¼'~øáמ‰ŽŽŽŽŽ~á™øáøá[Ã+釾÷ðJúá‡ßkx&~8~8~8~8~8~ø}†gâ‡ã‡ã‡ã‡ã‡ã‡Ÿ=¼'~øáÏž‰ŽŽŽŽŽþœáÊã.‡`üˆ¥á•"ñ#Ö^Yý?ÂÖðLüüüüüü;Ã3Շô>¥kx%ýð#´‡WÒ?Â×ðLüüüüüü?Ã3û%¢ß"ú5bÞ#è×oó*Á¿ƒѯøø—…+üõ·þOþýúãõ?óÈ«ô
endstream
endobj
12 0 obj
<<
/Length 986
/Type /XObject
/Subtype /Form
/Resources <<
/ProcSet [/PDF /Text /ImageB /ImageC /ImageI]
/ExtGState 73 0 R
>>
/BBox [0 0 7 1425]
/Group 74 0 R
/Filter /FlateDecode
>>
stream
xœE—A®ÜFD÷sŠ¹@~šEªÕ:×ÉÄ{'äþ@0ä#
SßOpSOjýóZïßüˤõèzÿúi½¿â¾®s=ñ¶}ųï÷_?_ëýùóç·wýðï÷×ïßüýý¿¼ðó¥÷zÿxé­÷×ÊÏH¾"oÈçó$·•lÁ>Ÿ¦ºu)fìºvêÚiø	Qj˜Q5T=´fT¯*¾~«‹W†ÕÅ«‹Ÿ†ù¬.Q]B
3ªKT—Ø
3ªËU]®ÕðWu¹ªË
3ªËU]®Óð»ºìê²Õ0ƒ¯‡ïg7̨.wu¹WÃOÜÕå®.w4̨.wu¹OÃü†«Ë©.G
3ªË©.g7̨.OuyVÃO<Õå©.O4̨.OuyNÜÍZlPŒPÃ+ƒë›ë{x%îÛžÙCî%÷"{Ë=æ^sϙ=ƒ6mLÚØ´1jcÕ¦=¼'~,Û|
ÏdÜƺyû6n,ÜüÏdäÆʍ™;7†n,Ýb¯¤k·k
ÏdðÆâÉ›7Fo¬Þ®3¼nôcù¶5¼'~¬ßö^I?°{
ÏDÃCÃCûÏðLd0l0t0|0"0Œ°³‡WÒ+ìYÃ3Ã0ÃPÃpÐðÞ3¼nÜPñCKÃ+¹©â‡Ö^Yý"²5<?"Âá‡ðCø!;Ã3ç†ßw|
¯¤_ßõû¶ß÷}ü~¨oýø!ü~?"Âá‡ü¯ÇýðCø¡ègýðC±‡WÒ?t­á™ø!ü~?"Â]gx&~?"Âí~höSs¯¤~è^Ã3ñCø!ü~?"ºÏðzÓ?":ýˆ¦~èìá•ôÃ=kx&~?"Âá‡ðCÏ®<),âä á•ÁõÍõ=¼'ƒ~¸­á™øáøáøáøáøáøáv†gâ‡ã‡ã‡ã‡ã‡ã‡k¯¤_ŸŒ|
ÏìÃQŸŽúxÔç£> õ	©Høáøáøáøáøáøáø᱇WÒ?üZÃ3ñÃñÃñÃñÃñÃñï3<??|kx%ýðÃ÷^I?üð{
ÏÄÇÇÇÇÇ¿ÏðLüpüpüpüpüpüð³‡WÒ?üYÃ3ñÃñÃñÃñÃñÃñß3\yÜ匱4¼'ƒ0~ÄÚÃ+«_àGØž‰agx¦úÞ§t
¯¤~"öðJúáGøž‰ágxf¿Dô[D¿FÌ{ýúMb^%øwð#ð#úu??âò¯Ða…¿þÖ¿óÉ¿_¼þH*«ú
endstream
endobj
13 0 obj
<<
/Length 1004
/Type /XObject
/Subtype /Form
/Resources <<
/ProcSet [/PDF /Text /ImageB /ImageC /ImageI]
/ExtGState 75 0 R
>>
/BBox [0 0 7 1425]
/Group 76 0 R
/Filter /FlateDecode
>>
stream
xœu—AŽÕHD÷ÿ¾ŸÊÈr¹|ÖÐ`Ó½˜™ûK#g¾LØHÍóêxvùï×8¾øÛ¤që<~7Ž·û×6?lÊÞó^×ñãó5Žç÷÷oG~óϯ××o~üú÷õå=þüµO­Ó´q|¾tŒãã¥CÇÇÿ~î¹6ãÓ+>½ Ï×ü[lÄ°ç«)/ͼ4F¬¼¶óÚ.ø"F£™
Fd
e­'YųŠ'Oxvñìâ³`Dvñìâ»`ü³ËÌ.S#²ËÌ.sŒÈ.gv9GÁ'Îìrf—sŒÈ.gv9wÁ'VvYÙe©`?~>«`Dv¹²Ë5
>qe—+»\³`Dv¹²ËµÆO8»ìì²U0"»ìì²WÁˆìrg—{|âÎ.wv¹gÁˆìrg—{ŒÙŒÁÅÕ<sr}q}5ÏdÃ5bÍ#kȵäšrm¹Æ\k®9³gcÐÆ¢I›6Fm¬Ú´šgҏe›æ'ŒÛX·1ocßÆÀ…›ï摌ÜX¹1scçÆЍ¥Û\Í3éÇÚíÍ#¼±xcòÆæÑ«·s7ÏÛýX¾-5Ϥë·µšgÒìÍ#'À°ÀÐÀðÀÁ0Á®Ý<!#l¯æ™ôÃ
»GóHÄ0Ì0Ô0Ü0ä0ì°{7Ï['7TüÐPóLnªø¡±šgò¤ÀÙh‰Âá‡ðCø!üíæ'}ï;¾šgÒ¯îúuÛ¯û~=ÉðCuëÇá‡ðCø!ü~?ä»y>^è‡ÂÍz&Ñ?4WóLúá‡ÎÑ<?"Âá‡ðCø¡s7Äá‡ðCø¡UÍzj®æ™ôÃ]£y$~?"Âá‡ðC×nž`úá‡ðC»ÑôÃíÕ<"~ø¡{4Äá‡ðCø!ü~èÞÍ'…ÁÁAœÔ<sr}q}5Ïäàn£y$~8~8~8~8~8~¸íæ'øáøáøáøáøáøáZÍ3éW'#Í#ëpT§£:Õù¨HuBª#~8~8~8~8~8~8~ø\Í3é‡~Žæ'øáøáøáøáøáøáçn‰Ž¾Ô<"~øák5Ϥ~ø5šGâ‡ã‡ã‡ã‡ã‡ã‡_»y$~8~8~8~8~8~ø^Í3é‡~æ'øáøáøáøáøáøá÷n®8îrƏ9Ô<"ƒ0~̱šgf¿‰ÓFóHü˜ø1ñcâÇď‰ÓvóHÕ!½NéjžI?ü˜ZÍ3é‡ÓGóHü˜ø1ñcâÇď‰ÓwóÈz‰¨·ˆzè÷ú՛D¿JðïàÇďY¯ø1ñcžþžÚ¬ð÷Ÿê3Oþ|ýõúd}´d
endstream
endobj
14 0 obj
<<
/F4 77 0 R
/F5 78 0 R
/F6 79 0 R
>>
endobj
15 0 obj
<<
/Length 8268
/Filter /FlateDecode
>>
stream
xœí][¯dGuŽÄÛIa'¢¼ô"8Òì©û%BH€±Ç$Œ™ØŽÄlǑ
ÁØQ~~¾oUÕ®ÚÝ»§ûœfò©Xaú¬®½jÕº~uÛý‡»ÅØ,ÿwPøïÉøgÒqÉ:çtxùÅÝîø}PJ¬þðåÇwþóÝï@·‹6^žîŸð€>ð¿÷ß©¾üôîé;öð酏Îÿ£'"ŸOîžã¿?]Oßúì?üá~tøÉ[?=ß]ðvQ:{{p>-Þڇ=""²zÃ,Nk¼ú_{| ž'f¯|èâý콟Þ=}û³O¿þòã.¥?]™CpKâ'{ÀÝâ':xµ~ÖTÆúÈKô¦Aþ²yjüêºÃ"¶qé:Yvj´w¿÷L§½¼û¯aD†#ñE<å$lþ{5—[C£`vº3½»þP§öOí[¿ËC5K,N?t‰‡ii#¡'±Ý×c5\$؜b<¸«S2—}ä—p§ïýôÝ·ðUu"§ÿþûßýê«/¿~ùUwŸ¼€;Að=sxñɝ.'ýÅ°dп	‡_Üýà¯Þxóðâ¿ï~öBø?µ :DpLpð‹'>3«¤ú¢¤~ORïäüžÈiúOÆс_üäw"Œ¬äŒEÄ5ò{BF®2vüViíŒ!¬Ô·w©Ïv©Ï÷ûûp«EÑcV‹òÊÒbem>ä°$¸Eý§{Ç¢ƒ‰A9eüß6ä%'¸ÇÈFÔ¿ølÌa	pG±Âð÷ÖQC»"£8²Fè'âàÈî`1íTȇ¨8ؤá¹ßÚ`@C$s°aÕÃôwQ¥%48؈ø63*»XØ%l¶‹³Ö"3"ç'Càh½À˙ïBJ‹
‰¹ÑäÅó—'á¨]:80j6´s'1ʞO{¨>eôèðŒNŠ	Î/Ú¶Ìn1ðqômõb­Ë	*-
Ÿ¤oŒÖëèÓÁ
Ã~"|âÁ[Ž™I
iÐ#hà­ Ef¾¤) ¨Ð>¸ŒOH6Gphä1ڃÉâña¨¾!}'cg=ÄM1‡' ZTÊaA¹P4…ÈL‹ÒœÏÈG6èL´˜	YÑ©ÿO!¡håŽp'$i‹4#æÆÓ
ʀwø¡%8,
™ -s¡Ó*lú¶	:sƒ"Öp°Áça4VE=(}3n"è,J
2ÊW9šA'Ÿ|0ÆmTèÔèÁÝ8h³˜d¬Œh4tAWcÓM5¢,àQ×܇ƒNüTò«û ðD8,Ä5GƒÓ#'MyõÉ ¹ÐY
ß®¾Á4ÄE¥wÚ¯nNk‹‹pß"™OÂ[èkè0Ó¡¬èà°F™004`Pp­ÚÐV¬@=pWZbœÏ·¦.¥`eÔöÎÓ˜DÄCÿT·‡dÀ*+ªYBè£B¼.1"`G
èd—¨%EÝueé@¿QšèjE¸/^ô`öjàY8¬Ö҈æªk5«V
©'qºÚ?A)ÁÓTðÕOÀÝâ	tßý)h0T	lšç1U 8êOW¥ù Ç䠔êË)-14$¬æõZ'í¬
1Sâ#¬çy¸Å¡}GyBŠ!ä ¸Dƒññ585˵¢{«!̉ãz"À7k¢žì)eè£%?HÓ"Ô vKga3šø0˜®‹ž »Î†T:h·'Ýn‡žœ»½z-Ûþà½2Tg†"Ò+öz38a/LÍ_jXsí$°U»½*öpiõ3m"«UÚ8a¯È=Zëö3½óT¿vˆÉ°ª€.¼BÛ\±²¹]Ld1'ÅDYLd1'ÅDßdaÜn'oCÆPüœíDYLd1'ÅDYLdñ˜'ÅÕ[c¶¶y'iÆçWn9
ûbæân#oGºÔ¸ã—ù$K"-§PözÏQG—×͞:ÌÂÁ}#ÿ²m
åâ%•üQ!õܵ7ÿÅ>—·Î4/;Lž¾ª*Ó«eyÿ—çgèßÚçþÆé¶V¦£#.ã鶖
ú>é)»º›-84$X¸Íw@>04ø	mîpM´8ÑâD‹-N´8Ñâ7-j
7îtÛB$h%­DÝgLŒ11ÆÄcLŒ11ÆÄßŒ'Œ
¼	b$6HÊz"Œ‰0&˜c"Œ‰0&˜ãú=¯nHîŽ;^ƒ2HÔWîxÙïxAîgsË«sÿÎ閗Ž¬Ñ†Yñ–›\:F†C4ó&×Dˆ!N"8âDˆ!>v"¨3Æ#vÛ6W†"Ššžç­'²˜Èb"‹‰,&²˜Èâ1#"Iï¾
Z^6wÈd[Ll1±ÅÄ[Ll1±ÅcÆ÷xÍa\¬¼<ðÞW¹Ü¼ÊõZ¯rÁmÓ"j'Ã\™1ô€›þÖÓwଛyk"'n'RœHq"'n3R4rQ1ü'á~€ƒCõ	+yºzb‹‰-&¶˜Øbb‹‰--¶0P;£oÁŒ"TšØbb‹‰-&¶˜Øbb‹‰-=¶¸v‡ËPl'¯©ÑЯñƽú÷±†.?¯n½Þ«[ȆEmsçê?ÂexFÛ¨ù#\"Nˆ8!℈"Nˆøè!"äà/ÂÆ_dùŸÊ̟ʘÈb"‹‰,&²˜Èb"‹GŽ,4D@úÑ7"…QAgóâÖDYLd1'ÅDY<jdqõ¶XÂm´}ÀÅ­0/n½Ö‹[ðXz¢]xȽ-›xoË¡pv.óÚÖĉ'Nœ8qâĉ'>fœH$³8$Ä<'}ÿŒJ§'÷u.óxõÄ_L|1ñÅÄ_<V|a£åÏ{Fw¾ˆ¼¼eò"^Lx1áń^Lx1áÅÕÛ\BK{"'%äŒ×nrÅywëõÞÝâ;ƒèƼtÐÙh÷ˆèi'ہͼ»5∠N€8∏ :"֎b‡‡¬?9þ'|Î&Žlæë	,&°˜Àb‹	,&°xtÀÂŒÜ"'߆,<|'E­'²˜Èb"‹‰,&²˜Èb"‹ÇŒ,®ÝÓrÎkz|æÕ-¸"€¸vW+Í«[¯õê–÷'Ù¾° §š‡Üëçe¼Å¸¨.óêÖĉ'Nœ8qâĉ'>fœèÉÄ<¬
›‡`Œ€ÆÚcȝË<[=ñÅÄ_L|1ñÅď_ ²­Œ¾
_0c):ïÄ_L|1ñÅÄ_L|1ñŵû\Þ"† R-$…ïé«·¹ò¼¼õz/oókzŒÃïÊ-r䳕"²z°-BFk¤i'zîíñy•)ÁÓ·?ûôë/?îEx8ø% 0ñ"P"Åü@Pb¢
E[÷G^¢4
òÂâ7ß3KáIÛ¸tŽGŒ,;µ?Ú»ß{¦Ó*n8_ÄC–#aóçØ+J{n}˜¦Oº3½»þP§öOí[¿ËCEšÈFC—Ž¿›R
øaËCҀöðŒ¤-©CBHYÒð%é¹@«‹ÉŠ"ó™m"ˆUˆh!"Dp;'è,V(:ðžŒ%}fº¨ú¢¨~OT¢íGYÈjL'n5ß*àqö!étüAÉ("(}¡QŸíR?ÜgQ
r¡AiŽkë7.iÒĈâ'Y·‰QlvW˜ü™îŠ4W(Žy¤H¢¢G["ÿ÷‹ñ03ëŠü×¢"¼$Ì)ÒZjÖFè0+ùù~ëŸï"Ÿí3ùVÕ0"a>ªB'ä3]žaòë7÷›ŸaþνÿŽ/ŽHœ°I\5þë_ÜÛ'êþXýßó4(1üŸûLží"ÿ£QÊMÖ{}Ú.â?
¾¤¿7ÐAÂöû<7þki»cçÈÄ[Éoï·>3Î3ãù!""ŸÓƳœ‹
§¡2JxÆnßß×áûûLþvìӆl=Ýo~†ËeÑø¹qžQ˙>Ÿï¼õÙ$=ïðAEþêýˆ¨®@S;,&˜š`j(¬pMÌ#æoNVvLzõ[ߏ±"ýa©¿¿ˆø~z­ù~ú‡A)÷8 Ôދ5rä¯LÞ67Ûã3ÓÉL'C":‰añ°©ÙåH¿.|÷R:qˆ¥Eëï"N¾Ñ‰cÍÀTWï¢ÁÜyÝÄU7¥Ã[¿ß<k¸ÁqéÙ§åãçœl]|Óøú 7:²Î&Õ|Õþ²\Qu¹ÍÐN•Çóë…ç}ٍqŸ"œ¹,z¨³Â:_24玘LKBÔ¥Ž^ßiŽ`Øz]m{¶OþÅ>"3¼?lKyZöÆV"ÞæK\ÕÆGK|§íßßæÝæiŽy¸KlÊb©	K€˜1^¾¬•Z»Xp	«?e	'za¢sGsn4†p?ö'^FI¢s»Ã_»|>R󥱿q¯Ögy¾+È9&uÊY•â·¼Ÿþê~ó;æÚ¿üêëß|þâãÿûêðƒO>y³åÜ£¾¨ÔÛ?þ'$¸Ñ[	ží®Î¹£€þ£Ým}¼rÌ䜩Î
úûûƒ~—ùóW¨â³U''þþͦNÝàûfõåŸïí£W)¨z§¹Ùk·¾ÿþ}ÔüAU¨mÜÛ}ƈ¾éY{¸É¾mVyŠK!£ß8NÙý7kBX—mpÀ½Z'sns®Ï}¿9ÇE_v¾Ò)£´î…b"&íiýؚy"&]xµÇ]"&»foq¸þvNƒßÙmý7ŽHçžb²YFEµèÈ^žÂ0™Ç¸õ‰IIt›iÌ>,p<m`PåªMVg'f:Þày/K9:0>ß"Ào ~~÷+>aø"'Uj°ÛƍȶJ¢36ªm«\Û)»íáÛv\ÚynòÇtÔ¬SK+µùV	µmáqKÓÛ´Qq¶€±<÷ðzT,ÀË |Œ
`<­¬,gR3ˆ¨™h¹ïxÒ~rñä¦wî"[Çó…[°\-uŽÜHÍú*@²J‡!÷!I‹@±ÈŒ¤•-mВµÉÊt
ÔÈ
¤f›¸ÉŸÂ¢Laƒi×l…flEüµ: •Ë¨'T_ÒiÁ:ép‰6Æ($ž³à´E)ôâêÃ)ñdf|Iñg~IÊ.!/ƒ†ÈHÂ%ð´D–‡Sp*·ž5p0š™TJϙçŠHsü­9+´¤C–vÑ*@éút"°<QG'uҒ7i†"©Ò·åÑAÒx"ùú´öŠg´¬#ë¢ð¬­Ž)x³Ð '´œRŠ¡*ÜÂÌñÀ•(±ÒR%« -f8ïA\'Ñ¡HKrÜè¥8†åYÀˆé7ÁHU)	Õé$‡"hù×Kt¸½œC®á̔"s''93¤r{_óYhR'¸hÖ*˜†¤ˆJ*k•Ód ºdèõÔ½õ¡´´È'4ŒjøÁiè1P‰y!U? F	™-¹UŸèùœ
Â5C¡!kKl!œƒ¾j"ŠHE ZÎþÉÑ`Îz`P`øªömx‹áƒÊdL큥'ê4\²Jžd؎§[´-49åÃ_¥æë]S}'!
ò
ÂËGQ®âq¼O\"$É*à{­ƒa«Â1.H–XýÄiHKA#6ïÑå{9€ë-§è'$§l2ÍJý\œM).tªä†,—dè,1ú(4ˆ±ººjrpwÉ
1À[KrÈÒ;ij)Ôµ~¡ñtP¬QâA"<àì\²<:HfI(:¡Dh"Ò"$‡˜ƒiá­¬¢õÞÄTÂ;HÏq…+m̯-9°%'YñXiá¨ùˑ‹§cäÖuZRHMpÉÀCrˆv;ôÁ€HªàeÔ a†ÎåÅòtѨ>]¢»¨'y@y£|S¸–,  ïÔrC1
cÞ"œJf)&$
&ôùЍ]iuØÍ1:µ"§'¢¶kƒ¸Ýtc!dÖ¦	³°"3óìÐFt˜ Ý8BKDdŽ4bª'Ù¨Œ+kL£j
ê…vñȆ‡ÏLܘˠڨbÂÕ¬B+N18@k9ºJã8ºTë{ã{MÈÑIëXF_®cÞø|SÍM…c5eoí™eÌj½1~O㿬sž'"=üì¤lâ¶(gq¹ZÐße\"âX틈Oa¦è\ F‰ÕÜ)$3é3xèP å¡d¡º,GÁ€§ÒR!Fæw쒜6EEàe	VÔR"Ó¹¤ZÃy¨œ!€Á²*hÐ%•à¾tÂãšÖ—þÕDݨ"
à°(ÌM)e~ìb*<Ëk­—™1ŽTZ#Hˆb!PŒ:¸Ju:X¾YÄ¢$æÆ؃ÛFŽ%*_[#¿WÌ
¦cãë­¢w	ˆ,®RD2†ïXžû¬0¾Ê'%8JÏN¨xQåÐtcC=PVæPªæ¼Ë²¿JYÍÔL*<ŸîÖLb¹s¬'•ðXÔ®šOð©'ñ¨g±t0Nˆ<³iRuò4]'T"‹	%IØRŸÃ¦'¥\m—2k£ˆæqXNJٖ£à3¡d.ԌäJÐ+JÞÂāó	N"¼äpš+›ú4©ª¹ËÙÔh×¥%¡L(é#zž eêòðі+x]Cñœ¯Î©&M¦.
ŽhA¡p;bËRZ"à4历d.J'Cjbé&C§bÉ\ŒݺÆ,T°²ò<Z\…Ô'¹" Ÿ.CÁ3Y2—ÏŎ%wŒâè£ÖÔ´žÈ¹	»æ."ZÉ]°¡n*2+Ód]"'Tv%w¹,O%‹sYj?qŠgm=°¦Lò.§§ÂH\Kz1©Î8ɈgxÓá	üËÁõSÉp­ T½—â<ˆ¸Bªâ±]¨eê*Ôbn(‡ê³Ìr`Ä'¨»Üxää­P'J,uÈ%'0Ö#5@['à_˜dd
ø8¿pÈ
çÀ…ì ™_CÀ\ÈHê¨O¸ò¼ãtã'Iôý"'ò­"f¡æˆ|ùó˜•n&T"Kø'é'Iæaí1'@gH•
}£˜:z]iæÀªÞÊ-R'œ`m"IRžóôÒÖe¹ñÁ´.å:äošÎåF'ÐUâ̑‡¹'dI*-5SsºëYz…HOòGNی'¹¼'9†»¼¾´°áí¸ÀªΒø³äÕ/ZºÖ|W
åõRÄè`Ÿ×Z‡\é
=—'"©ù@•J§0›@æ+¹ÒÑoÌX•-ºÈҘÅ3[Z¨¨ÄHæTJ'³eH®lþÂûä*©`TK'‡'­¤}ò÷<â*
'Zå€)F©1(bLȕP¥–r}[±æu',"3®œjñÛJE¹áuN3c.¦ºL±x¬žzÖ±¶Ž.I¥/Uê3ûc}"3U®"59dºÊ'‹b
"ÆÈYRZ–`൮ŽõP*<oW 46їzÊB'¢ªsÖR¨1#ļ߻bà՘Q @UñÒ½•Ê¨X"K9$5QF@åÃ~ŠafÓ¼ÌÅ
:{Xd[šî1mÙR_¿T%óȟáG,/9ÆËr
©Ù#ieՁ
¤,óöËÂ"pfÊä`QƒD<RáGšT‹,¦u	`δ9aÙ³ò&˜Ç(ÍÆ9$_ZѬ¤#äï*‹ÈY UÄȞʢ–˜sYk*`R5áÊÞüÏ%á¶Ç'ל;j˜ð‡qöˆ)¢©9žˆÀrgãV\®j†œFÆwP%åOõ™ÞÑ÷'Þ†nt¤døœåÍ¡c"pc…#ؐ¹öÄÖBhiw×w>¿ëÊó'ìzWµ§œF¹ŠX©çÓ2Š:.C®#æLnÐPUÖnÍɢϪÎfQ|Õ{+"ÅHÕFy­"ŢŠšÉ©ßÈcp'JÔÍOŠC5-¾·aÚõH€æÔa«ûoÕbåX5²¶êªA¸Õl‹Ø#3´ðޘ¬&'mÏ%'' w֚UV¯·¦ VдâV9ñY'ÅQ˄˜ÞjY©
9È¡R¡3ؒˆ"®}ñŽ–\'"*Ŭ†¬,jräí¼Ä×ôE.ôòi(³9Cªãí4XÏ*Vo-1cF

ٟësœÒTVÄxåW@%UZV¿܅VÇØÖØÃ@këiÄ)cˀ'åӖc ÖÅ·Û¾y	OA/ƒ"†·íx®hq¼ðm¶Ãæ•FâçQAFê,þ HÃ}ŽhÍVå ¢; ŽÁ8fLjæÔÜåéڒ‹§x}àȕ-›*ÇÚ7"ˆ+÷¡>]¥L\ý¬ƒáÉ8%}Ôr'Շ¦²ªÞJŽ¶.ÑV52/%®vu…g"D[2.¦•ƾ¬UæbBž8Z7Ænn1¶lî3p\mÓwwÉ.euÝÍhª"çí¸K8P]A5lò Ç_G
¯'FÓØîÄv‰zþ&ØéZN£Ê"©¬lFpÞÀM' ÛËIe¡Y"eõ€([¬¸îÅ«'˜¢9ˆ Ó6$u~<¾ÁrBCšqÜþ
s]çò'h‰s^¿pƒ'|7¹í˜Q¡Êê)`çÁB s¶UZ"YÎVy97r¶$›#ÑZ9çXÇX×°8	uãŸ[ð¾Û´´.;Ó8š2G5Hºõís<ëT®Bk:‹‰ç8.&ÉzõfØ~ž,Áõ¸n¿Q¤âR0ïŽ*œ¥•‰Õ8qLjñÔÜåéºÆËÄ&¹r"EUø§çÁÊÒuY|M\<°UpY–']_lƒ‰¼å˓n6WÀ×K|ZÄUn…pÁ¯©c"¢B]À(úŽ\dÂ4º­ÑË𚽶±®ïÆbÁ¾°Í˶[7¯[6ï96?ÛöÝ<r²9î0"æáÛ1·XµÓbfÔb‹®­¾[Ž–Ù1àNd—˜ô»+#•îeõѤ$kBU>"2qò<ó,3LT'Ì…€F|¨‹yžiLËl	sSZk™ÔÀ«Bˆ@H;څ"o.T ¥UŽXä´1úºžhyÍ
Šâ'Ô`e'Dx…L·  `ʞÚr¢K<Z#7RàI¦L°ô
ã¬#Vˆ:±MÜsӖSéÄ¡\9;Ž\šßJ€Ù*À摴 ÿ›Í¸lä)À΍
@å†íFY–{αÌ»^AåºN>¶'åv)ç	£Éì®yíŽ3Tµµœ§PMŠÂ—F2€œìRg•ƒ*±ç:eæF›ÜßOrskPƒæÖoô*­Š,:Óܯ¶Lٛv5J¡Žòz‹n	¾`E4ê6/VؙØd°¯®¶£/4¢ok6Åo6m›‡m¸Òe»J`Û
{ñÜQÚÕÇÇq­áp¤"5v6*ëq6j·GåÖ=†ù=ï冚7øB‡¶rúÅú'§ ÈWÊ1o
Ñ[b$Îy•'òb¡š\™üsÑ#ˆ"'εKÍÉ·¯üZ²°ò'Ì·ªˆéX*ʺ/[× £Ö.V=AêWÎr=K¨W=ø›!º©ócnER¹CÆ#Éu™Q{-é(¾Úšºh
¡6¨r; -B`Ô\…õm
ˆX†çm[ñË–#-$Œ'ý{¾^ãXXÇ©"F3ŒT
T¤G
^9謼õG—êU½¤ruáÈ>ó=ii´©'F®Ä¾ÎPÛ5)Ü6ÌjÏG7)",ڌ§þhìMQ=U•n4ÚÔ¤ýf«©šYwmï×aqM›æKnÍñ6=w/¤ì½ñçæýGÎ_#e(-¦6!Õð$þJ´ë±9Çпæþ˹pZ%&j'«å¬Ö«ïÁ¼âê5GWdõ¯^<ø^9;©	MûeÒz;r-\õ³·ïՋZ9®åoO'ž´®·`ƒ,£XutKá¤ùó}ò‡ã­'sÚ254pã÷*e½ò.ΩÂøª®1sÕQx#——¸M´sžÅŒƒ\UòÁýTõa;K+ï_:ºBqB~ã
"ØՒ‰7¦OÈß¹FƒDœ¢é{hp¼^®¸¹ö
ÓëѝÝ?ñ1mƒÉu–Û¦@â"uéŠËë×ë^Λ»á×·÷UòwûcÿöUym¦·ÀÇÉ]qaöÏ6"«ÂbBâK·¸'÷—3"ïÞsdyjê/gÿpÏ!8¶pÍëoþlCøÇ{X…'ð_¯#½ñÐp~^ÓÙÓw¿øͧ÷[æùhx<ðD"å—+¡~ýÙíé§ôÇ'e$GÌ֟]"ü×ƆPÞi£æ6ÑÂ¥MÝ?\ä·¾ßΧ…P–/ú"«ó­€÷çfÖdiQŠoc»Ýú+®Ï™)Ü2X³¾ËIóTŠ3¼Ã~ƒxë+,ªyµá&vë{&ø¦S`tÆ3\99«s°Nqã"¤‹¼Öëð|9Grtö¡>gV"â¬â:«¾ÍçÌ–¯çå;fnÐÚ.ðՔFßær=x0Úc"Ëúë½ìnݗ›]ãSRŽ4‰âøžª‡p[Ã!(yçMÌÖXà¯w$8š}°·Ù5ß
"«ø|ç¨áËhïëmÖõp1¦ý ;ë÷ç	‰Î­y3³åIÞ°[c!ÓÝW,na·†BL\såõ§[BË®ÑQ*³w7Ŗ]ƒ!ñdïkÝÀÍõâ <r™êçÖPàk–Ì[xȗ(Ó燈ÖƒEhÉK»‰ø´·òºä{󳝟…æfÕ-ü֘@ÆC¼öàtî|gÆýú,o%敌‡é.t³fÇi)ߑ¢xj^Ž£Ü›_‡K!¦¼‹·ñ[C'Ç,7"嶴âÛعƒ	 3'+4ÀeŸ2ü¸"¡¦
endstream
endobj
16 0 obj
<<
/Type /StructElem
/S /Part
/P 8 0 R
/Pg 7 0 R
/K [17 0 R 18 0 R 19 0 R 20 0 R 21 0 R 22 0 R 23 0 R 24 0 R 25 0 R 26 0 R
27 0 R 28 0 R 29 0 R 30 0 R 31 0 R 32 0 R 33 0 R 34 0 R 35 0 R 36 0 R
37 0 R 38 0 R 39 0 R 40 0 R 41 0 R 42 0 R 43 0 R 44 0 R 45 0 R 46 0 R
47 0 R 48 0 R 49 0 R 50 0 R 51 0 R 52 0 R 53 0 R 54 0 R 55 0 R 56 0 R
57 0 R 58 0 R 59 0 R 60 0 R 61 0 R 62 0 R 63 0 R 64 0 R 65 0 R]
>>
endobj
17 0 obj
<<
/Type /StructElem
/S /H1
/T (Change in Fidelity Over Distance With Co-Location)
/E (Change in Fidelity Over Distance With Co-Location)
/Pg 7 0 R
/K [12]
>>
endobj
18 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [17]
>>
endobj
19 0 obj
<<
/Type /StructElem
/S /P
/E (1)
/Pg 7 0 R
/K [0]
>>
endobj
20 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [18]
>>
endobj
21 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 1)
/Pg 7 0 R
/K [2]
>>
endobj
22 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [19]
>>
endobj
23 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [20]
>>
endobj
24 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [21]
>>
endobj
25 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 2)
/Pg 7 0 R
/K [7]
>>
endobj
26 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [22]
>>
endobj
27 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [23]
>>
endobj
28 0 obj
<<
/Type /StructElem
/S /H2
/T (Adjacent)
/E (Adjacent)
/Pg 7 0 R
/K [1]
>>
endobj
29 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [24]
>>
endobj
30 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [25]
>>
endobj
31 0 obj
<<
/Type /StructElem
/S /P
/E (2)
/Pg 7 0 R
/K [10]
>>
endobj
32 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [26]
>>
endobj
33 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 1)
/Pg 7 0 R
/K [4]
>>
endobj
34 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [27]
>>
endobj
35 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [28]
>>
endobj
36 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [29]
>>
endobj
37 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 2)
/Pg 7 0 R
/K [9]
>>
endobj
38 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [30]
>>
endobj
39 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [31]
>>
endobj
40 0 obj
<<
/Type /StructElem
/S /H2
/T (Offset 1)
/E (Offset 1)
/Pg 7 0 R
/K [11]
>>
endobj
41 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [32]
>>
endobj
42 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [33]
>>
endobj
43 0 obj
<<
/Type /StructElem
/S /P
/E (3)
/Pg 7 0 R
/K [13]
>>
endobj
44 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [34]
>>
endobj
45 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 2)
/Pg 7 0 R
/K [5]
>>
endobj
46 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [35]
>>
endobj
47 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [36]
>>
endobj
48 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [37]
>>
endobj
49 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 1)
/Pg 7 0 R
/K [6]
>>
endobj
50 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [38]
>>
endobj
51 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [39]
>>
endobj
52 0 obj
<<
/Type /StructElem
/S /H2
/T (Offset 2)
/E (Offset 2)
/Pg 7 0 R
/K [14]
>>
endobj
53 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [40]
>>
endobj
54 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [41]
>>
endobj
55 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 2)
/Pg 7 0 R
/K [3]
>>
endobj
56 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [42]
>>
endobj
57 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [43]
>>
endobj
58 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [44]
>>
endobj
59 0 obj
<<
/Type /StructElem
/S /P
/E (4)
/Pg 7 0 R
/K [15]
>>
endobj
60 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [45]
>>
endobj
61 0 obj
<<
/Type /StructElem
/S /P
/E (Simulation 1)
/Pg 7 0 R
/K [8]
>>
endobj
62 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [46]
>>
endobj
63 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [47]
>>
endobj
64 0 obj
<<
/Type /StructElem
/S /H2
/T (Offset 3)
/E (Offset 3)
/Pg 7 0 R
/K [16]
>>
endobj
65 0 obj
<<
/Type /StructElem
/S /Figure
/P 16 0 R
/Pg 7 0 R
/K [48]
>>
endobj
66 0 obj
<<
/ca 1
/BM /Normal
>>
endobj
67 0 obj
<<
/ca .39
/BM /Normal
>>
endobj
68 0 obj
<<
/CA .6
/ca .6
/LC 0
/LJ 0
/LW 1
/ML 4
/SA true
/BM /Normal
>>
endobj
69 0 obj
<<
/CA .251
/ca .251
/LC 0
/LJ 0
/LW 1
/ML 4
/SA true
/BM /Normal
>>
endobj
70 0 obj
<<
/Type /ExtGState
/ca 0.0
>>
endobj
71 0 obj
<<
/G3 66 0 R
>>
endobj
72 0 obj
<<
/Type /Group
/S /Transparency
/I true
>>
endobj
73 0 obj
<<
/G3 66 0 R
>>
endobj
74 0 obj
<<
/Type /Group
/S /Transparency
/I true
>>
endobj
75 0 obj
<<
/G3 66 0 R
>>
endobj
76 0 obj
<<
/Type /Group
/S /Transparency
/I true
>>
endobj
77 0 obj
<<
/Type /Font
/Subtype /Type0
/BaseFont /AAAAAA+ArialMTPro-Regular
/Encoding /Identity-H
/DescendantFonts [80 0 R]
/ToUnicode 81 0 R
>>
endobj
78 0 obj
<<
/Type /Font
/Subtype /Type0
/BaseFont /BAAAAA+ArialMTPro-Bold
/Encoding /Identity-H
/DescendantFonts [82 0 R]
/ToUnicode 83 0 R
>>
endobj
79 0 obj
<<
/Type /Font
/Subtype /Type0
/BaseFont /CAAAAA+ArialMTPro-Italic
/Encoding /Identity-H
/DescendantFonts [84 0 R]
/ToUnicode 85 0 R
>>
endobj
80 0 obj
<<
/Type /Font
/FontDescriptor 86 0 R
/BaseFont /AAAAAA+ArialMTPro-Regular
/Subtype /CIDFontType2
/CIDToGIDMap /Identity
/CIDSystemInfo 87 0 R
/W [0 [500 0 0 278]
 11 12 333 17 [278]
 36 [667 0 722 722 0 611]
 49
[722 778 0 0 722 667]
 70 [500]
 73 [278]
 76 79 222 80 [833]
85 [333 500 278]
 89 92 500 111 [496]
 250 [531]
]
/DW 556
>>
endobj
81 0 obj
<<
/Length 354
/Filter /FlateDecode
>>
stream
xœ]'Ënƒ0E÷þ
/"E"mi$"""±èC¥ùE*g'¿¯ðÍCêЙ‡}/3AVÓ;|Ú±.Éñ¶7¥y¼Øšø™ºÞ0©xÓ×îFþ]Õì8–×ÙÑP˜vdIÂyðE]?;{å«}3ži͂ېíMÇW§¬\³ ¼LÓ/
d,MyC-²·jz¯âoÛ
×»ë攕ϊïëD\y–PS
ÍSU"­LG,Bˆ"'yžç)#ÓüËK¶s[ÿT֗‡)O"P"]HJÐ+hç)ŒAЋ'¥=i	B¥F¥F.F.Ê<mwžâ|'wÈå{ðboªvwOO¸Zà$Êå²`@Å(AP‡>ÂU¨"¹0º›[>''rÞÃÚ5®ÕGáCç÷>Ì`gFøsË4–­yŒº¾XKÆùÕòã]Ûzlß4NK×òüMÁ¶ˆ
endstream
endobj
82 0 obj
<<
/Type /Font
/FontDescriptor 88 0 R
/BaseFont /BAAAAA+ArialMTPro-Bold
/Subtype /CIDFontType2
/CIDToGIDMap /Identity
/CIDSystemInfo 89 0 R
/W [0 [500 0 0 278]
 16 [333]
 36 39 722 41 47 611
50 [778]
 58 [944]
 71 [611]
 73 [333 611 611]
 76 79
278 81 82 611 85 [389]
 87 [333]
]
/DW 556
>>
endobj
83 0 obj
<<
/Length 326
/Filter /FlateDecode
>>
stream
xœ]'ÍŠƒ0€ïyŠÛCIâ_)ˆPtûú}MF7°ÆӃo¿˜±]؃'oÌÌ|qÂʦjŒö"}¸Y¶à頍r°Ìw'ö0jCDD•–~§°Ê©³"•MÕ®‹‡©1ÃLòœRö	£^¼[éáªæŽ"½;N›'ne{$¬½[ûO9)
ª` ¬|íì[7e!íÔ(0^ûõt+Û¿_«h#g‹í$¸ÎŒ@rÎ9/h^×u]0êßw±§õƒüî\Ø4ç<âÅF'#U¢$P".HRTŠ#¤é(=J°J†UÌË0/Śg¬™–H— ¾;¦ãç	YxÅ»RtF'›a0©°'Sv¨œ½`0}(ƒh7ÀžÛÜæý'¼;ƇK³DxÞ;Û-k{~!‰¨
endstream
endobj
84 0 obj
<<
/Type /Font
/FontDescriptor 90 0 R
/BaseFont /CAAAAA+ArialMTPro-Italic
/Subtype /CIDFontType2
/CIDToGIDMap /Identity
/CIDSystemInfo 91 0 R
/W [0 [600 0 0 278]
 54 [667]
 76 79 222 80 [833]
 87
[278]
]
/DW 556
>>
endobj
85 0 obj
<<
/Length 282
/Filter /FlateDecode
>>
stream
xœ]'MkÃ0†ïþ:¶‡bç£í
!0\9ìƒeý‰­d†Å1Ž{È¿'³v°Å#ë}-$.ëkmMþî'Õ`€ÞXíqžî^!t8˒´Qa#ºÕØ:Æe}m–9àXÛ~bEÀ?p0sðìžõÔážñ7¯Ñ;Àî&›=ãÍݹoѬ,Acϸ|iÝk;"p'j6˜°n²ù«ø\BJœÄnÔ¤qv­BßÚY!"%UUU%C«ÿ½çQÕõê«õT•P'Šr¥ìDẗòœè"D''.ä»9d¿~ï"(JŽ²M[Eß4ZHJÏ1ùDáœo¾Ñim}ñc.êî=Ú@{ Y¬S0«r"[Uëù¿Œþ
endstream
endobj
86 0 obj
<<
/Type /FontDescriptor
/FontName /AAAAAA+ArialMTPro-Regular
/Flags 4
/Ascent 726
/Descent -274
/StemV 94
/CapHeight 716
/ItalicAngle 0
/FontBBox [-222 -321 1006 923]
/FontFile2 92 0 R
>>
endobj
87 0 obj
<<
/Registry (Adobe)
/Ordering (Identity)
/Supplement 0
>>
endobj
88 0 obj
<<
/Type /FontDescriptor
/FontName /BAAAAA+ArialMTPro-Bold
/Flags 4
/Ascent 726
/Descent -274
/StemV 156
/CapHeight 716
/ItalicAngle 0
/FontBBox [-167 -302 1012 939]
/FontFile2 93 0 R
>>
endobj
89 0 obj
<<
/Registry (Adobe)
/Ordering (Identity)
/Supplement 0
>>
endobj
90 0 obj
<<
/Type /FontDescriptor
/FontName /CAAAAA+ArialMTPro-Italic
/Flags 68
/Ascent 726
/Descent -274
/StemV 266
/CapHeight 716
/ItalicAngle -12
/FontBBox [-262 -320 1061 936]
/FontFile2 94 0 R
>>
endobj
91 0 obj
<<
/Registry (Adobe)
/Ordering (Identity)
/Supplement 0
>>
endobj
92 0 obj
<<
/Length 7771
/Length1 12612
/Filter /FlateDecode
>>
stream
xœízy|[ŵÿwFÖfÉڬŶdûʲ-ǒ¼H^Œ-ˉãx·Ý8‹Ø‰³›$,	)¤…"ÔÐ%–ºÿºp
…š=a‡:¥.Д=
k€x@<ïÝ+Ù1–¾ßç}~ü>oÆ:w朙9gÎ6w1=v@†¡ÖÎbÿJõ} ?л ¾96xÏP) ëä/¯Xß7ôÙ§ò{š`tÅ[8ͯTwI‹òêÊ¡UëWènü+`.'oYÕ·y*Ø|@»jÝ֕+/±|d¦uƒ}ý
åÛd€ŠÁÁ>ňL	¹r×o¹¨­Bq1<ÈÞY·qEßâ½}¿a€|º¾ï¢!:¬éˆ
·¡oý@öŽêkz/@nÚ¸y… "}hÓÀÐ/þ´ý#@UÐ"P¨Ìôõð9:¡D;'¤žâ®ò'oRawˆë}M!}~â=<.û"å°|Ù{ÒÓËç†k/žX´L<
ì"á™ã#ÃÒõä'^–3ñ€ì=ÙõÔ ‰™ITG~9'è0hŠ_ÉRøI%@5r*Ñ*$<eskK+9îs'íRËW‹4ª¤c¢V ͂L'N‹$ü@¾"W€Ã¡¨B-êрVt¢«°q¶~N"V)@Jã"h@:ЇXu؄­Ÿƒ1öÚ7Õ¸~¾±ˆ†"X$Jž¤p	M´	ÒðûD›B‡Ÿ$Ú2Iªx;iÚ9Š›h+ ›°}X‡ft¡
›°>t`«p>Ö¡›°؄ÍXØ¥'JÀ¡çKû%Rm–FmÄlÅÀ¡ë%M®Æ¬'ú°E˜9;'ñç̄%(Eù9'ü³ñlĶJÔUĖÿ²ç¯ÁM­Â¡ƒ',_•Nœ»	CìÖÄ.‹À¡ë$NgWÝ,õ°YÒÈ@?Š:m–Ð'òe#R´¨Ø))®¦ «f§ÿ
øoÙ
üÏ®øe€å‰vbX"~©½èœqÝèB;æc>1ÑDo.ŠÔÿ?–ù¿QÈjöñT§îkk.™ª?ÄqÇIÙC'CÔNíô;_©·Ò[é)™W敵S7Én•êIÝÿ¢>–ô˜\!Ÿ'¿Fþ'…_áWÌWlSlS\©Wj•õRݨ|\EUª…RÝýoÕÿ·~µª+Âìï/[mŽçþlµ9.Þnµ_¼=ý™£V›ã'­6Çú!«Í±n£ÕæX»Áj_»áÒM[Î7[«Ö˜-Ž•«ÍÇÀ Ù>0¸ó¼ŒôÍÖm'tçÖHºóúý
ρýjÏþ½ύ»Užkv«<WïVyöìVyvïõ{nÚK<û÷Ïu{•ž}{•žk÷ª<ßÛ)÷\ºSîùîN¹çòrÏe;å{¥%­Âb)·˜Ê,ú€Eë·¨K-Š‹¬Ø'"K¾[WàÖzt^>Ç¥Ëué³²u\¶þÝ÷Þ×ê
F­:Y£U(UZY'\Bµv'™'¦ÌH±l)¦$sŠ7X,æÙ¹Áœ Ì
ڃiAKÐÔÕAEPD°-ÐESšºê"T҄¦Î:!ài•q'ßÓ$¨Ûzb#"ü€î%è'vRt	¦È¢žØ(IÉ;íwM½;¿Ï{<™BSgLؑÉ~±ñ£LM'¿]°»ê<ßTF
ò£Ba´OðF{마!AÁØÔ¹)\ϟ¥iB¨©ó+FÔâFÚ:êšUG" jë2\uMÂãMBE[ uՍéŠï §Ä³ '=¬ß]š$ÍÒ9üe¼¼x¥^ø¨©ꅗzÿë6Ž/œ~ýW…^/Ý·€E€E›Ô^¿þÓ9GÑ*K–ród¿^ß7ñúÚµ¼È—öt
nêE.õÂM¬PQ/r¤ÇÁ1öìd[V‹ZêE=õÂ5¥f"É)d+ŒÔ‹:rêìKNÁð#××rªÿ©µþ·üÿ]h*T b´øTÅ 'ŠM@
5;ƒd$³/ †}-´ì¤HPûzèÙç0HÐû&ÙgH…‰}3RÙg°ÀÌþVXØg°ÁÂ>E¬ì?ûHgŸÂŽtö	È`#vö	²à`#YìpÈf§áÇN#Nv.8Ù)ä"‡FrÙ)ä#'['Èg§0nö
1ƒ}f°àE!û>xØ('`1¼ì" ˆ}€R³àG1{"²÷Q?{å°÷Q!µ+QÎÞC*Øû¨–Ú3QÅÞÇ,T³wD%{³QÅÞE
f±wB½ƒ0f³·Q‹ {u±·A˜½…zÔ°·E-;DØ	ÌA=;¹¨c'Ð(aæI˜&Ìe'0
ì8š1‡Gæ²ãhE#;Ž6ÌgÇю&ö&:0Ÿ½N´²7хföºÑÂ^Çt°×±mì5ÄÐÎ^ö¡›½Ž,`¯a1²W±Dj/ÅBö
–I˜^ÄØ+èÃbö
–£‡½'èa/£‹ÙËÀöw¬Ä2ö2Va;†Aô²câ;†5XΎa­סŸÃz°¿aV²¿a£‡°Š½"ó°š½$>¥°±kØK؂µìñ©‰½€$x!6°¿â"ld/ˆO>lÛ0ÄþŠ‹qÇvlfãø¶°q\'-ì/¸ç³qìÀì/ø6.dãø.bÏã2leÏãrlcÏc'.fÏ㻸˜ýWà[ì9ìÂ%ì9|—²ç0,Á+±ƒ=‹«ðmö,¾ï°£ø.cGñC\ΎâGØɎb·÷à
ö®Æ.v×à{ìiìÅ÷Ø3¸ÃìiìÕì®Ã÷ÙìÇ÷ÙS8€°#¸?dOáüˆ=…±›ÆMØÃãǸšÆOp
Ã͸†Æ-ØËÆðSìccø®ccø¹ýìOø%°'ñ+\Ϟįq{ÿ7²'ðÜĞÀo%ø;ü˜=ŽßãfönÅ-ì1ÁOÙc¸
?câvü'=†?àìQ܁_²Çp'~ÅÅñkö(FñköîÂoØø¿eàüŽ=Œ{%x~ÏÂýØCx#ì!Ä{‡p{âvváìÆìÁìÅÙ!<&ÁÇ1Êâ	ÜÍÀ"¸‡=€?Ip÷²p÷±ûñîg÷ã`÷áid÷ãb÷á(d÷àY<ÈîÅsx˜Ýƒ?ãv/žÇ£ìü²{1ŽÇØ=ø+ž`wã<ÉîÁ‹x'Ý…—ð'v7þ†1vŽá0»ÇSì.¼Œ#l¯ài6ŠWñ4û#^Ã3ìxϲ;ñžcwâM	ǟٝøžgwàþÂîÄ[gwàmü•Ýwð»ïâEv;ÞËìxc·ã$Ž±?àüÝ†%ø^f·á^a#8×Ømø¯1Ÿàu6'Oñðx"	øǙ€Ïñv+¾À	&àN°[1·Ø­`x›ý>¼°gßÝÕÙÑÖÚ<¿i^ãÜ9
ÑúH]m8T3;8kfuUeEyYÀ_ZR\äóz
g¸óór]9N.;+ÓaÏHO³Y-æT"Ñ ×¥h5Éj•R!O'Q/IÒ"±è!=Ò+h]õ.'h[N60ٝ.#(æ}‰Q'Ü# µI0·ÅF®â…çÜ!-',Ïð¡S€©ÙÎE…¤<!)Ï5¯¯_(èˆ9]†çíStž÷y…ŒHÌé´4O y',OåÍëãúC[Ì)$L£€¶˜øe¯V9íªœ¼]@GLȚìòü×	yÀž#f6ŒhÓ#õÌ#о*À";YA¡À#Ð<ƒ€ ´ŠbþP ©±40}™…8í媯ÑA´+Ú¿ZH¬é=«Ô"q•:¹an¸#f؝NIê&áñö؈&9âŠ$ó>/$F'5WD#"­kh"hkˆÔ ÚèÌ
UŠÏ+˜Dy£âo¾²W y®z§Óéó
©g)£ìàUÓILžÉVj¼BPDe\nµîp%7â=8|Õ¨Ë{=Ú~Wß☠ëã}ÞÈò¢ƒ]'£©mQLåEÅ_ï 'Ú»^¢õ¸è 7ìªiƒ½',ÏU/ZýKøþÁ^ÑOH¯«ÞçԑØ΃vÁ‰]Œ!ÅU/¤l{Ý.Ž¦­æÄîððœð"öØtªS"<ϧù¼ÜpÔì­÷y£kêD›OÙMrÇÆ~É:á+û8aÇò5qçë»j2œÃAû±Óît:¢y¤‰	Uö÷®E^Ó'n3º†¾r@ÚêUÒ֜N;]S/þĉ\T@·Y‹º¢grî>Nå;×éÒ=âÄáá¨(b_ÏYH÷œ•_
»‡4/""»¤º$pQ!ÜWÏ'P‰‹Äi"¥·žçq»Ëò8A™w…¼ÈÅ
‹+*ó³Çà|Øéóôy›:bÑz»´{Fbgø¿O0IaüŒ](É#ù-'o6¼Ëû¼MmS"HZSGl¸ø]{\ƒM®¦ö¸N'Þ®x|Ó)¿p:ùÄx'çìÃiöÃñ¶@:ıN§½ÁÕÐ;<Üàâ†{‡ûFَå.ÎàÑj‡‡¢½œ"%Hß(»ûJ»Ðp/zÉLїEßlèhRÛ{DS6pƒ}ñÌr9«ìNãԘ¶FNĤ Œ
)&‡
ïø¼'6sÚ¹1²"UvÁP%†4' ;6jÀ
É¿%Ð' 3&P»U2>/ºº3¡.»sÒ¹Ä$ٞÀò>¯Ó)Æە£a,÷yÂŽöX¼Ïa¹ý6"‹=¼@{EÊÁIŠ¥[¤ì˜¤LMïu9}Þ4ñýÅ¿ôÿé¾?lt™¸êbÉRnîvÅFÙ§U'ª*á©'˜ÌN-j—‰­dËÀ›Gš(êD(ð\ÜÓ.Áàä'ØA{çF&âó
s=b"Ñ<ÃÓ®'ˆ˜ha6$(«ˆGª@¤ü/³U	$uʕ¸èpoÂצo+qZô~ýބ¤<ƒKÐ~l7š\âǤô—Hëy
bÜٝñóxA'ænA÷Ž|^Á‰qé
h—\"-p½õRÊàíÓÑ£ìåÞz1EŠAĉ2ǝœ·Çý_óyÿ]ßq¥]øöUüàLŸW:}^®\ ½R¼tÅZª²'bJäÕ(nåËô)-NŽn¬—yØà<dÂi‰ÐþŠÖ›º¾Ô›ÆO¢UM%®˜Ðà™\?ޟã±OïÎ=‡Ü8I†@óŒ¢ë­á¤Ø	÷&–ý¡=&"û&9wľeß&®dBiêªóyG(êF\dWûH˜ìê\»Ëp»ºb·QB#½uüH.ÙÕ»‹Â–ŠX)v8±#®Ô»ª¤ñö»ÂÀ‰š$!¤þŠQ	§šÄ¬¥qœ!Î(_bŊѤ8%<9:	+FUqÜ	'•ˆ
	'Ëê°:¬¥)Ô¿w›<¬º›j'Ûµ$…ØGvÐH‡"%;FÔa{|ĨI8.á®î³¬»Ån×"…Ø%Èó|X|ÞhÚ «©=æâ¢\¿n‹mç‡{yÑiv4Ò&Ñ@=bú¸Œ'i_à=b2|C|#'ß7'ãt?dP@
-ô†5z¥2E¥HNÖÈ5w³"P³"á:…˜´•A«'Söû«ªB4šª	"–Ì F§ÒiSº•6#qºÉñ‰<òâü‰ûnɼù…[&~B"7ÓýÅ~8áøð#òƙ>A':Ž$ߞäP"B¥%©ælâ*"åe•½v7	µ-ù]¨xVIzç8}ñ»ÿhßþ3ñKh.+":ÍôÙĬPº*ÊËòÝ+1,ií™77ô;"»øôÀ»'v=wÑâLñ=é}è‡šÛébB(ãpiIÀU¸¯¿¿ ð±Sô'a…-¬Uènàé0ßÀC‰i!Oi	ñ[-f…+ÇXV!3[~'«+GA¬›.ºpÓ[[2ê›æ×ϙ7¯ž¹stô²þö{&ö\½gÏÕ®Ú"~Ÿ%J¸?&É Tí畣ìäJ¥,Mdª.®òM¨.-!£Ë¨#ÊòBjªcÎކóè'3¥´${–¡ÛÙ@NÓ#Ȃ'lQi»]"¦ÓìçuiH›&¶¸bZqÀ(ø³ˆÅ¬#JQ:-βŠÊ߄Ò]Cˆ¥~ ¢º#§'eîEÍÍ1ÿü™Á6²H½)ã+ªWv"—Ïæºf_w¶VÌiœ›<°^vŠz>"ÃœÁh4+¸lçø1Ïqf¤˜oàSÒ=……n¸'H+L
'vMÕ&QÌI•q9]9ùîÊ,ðאò²""ÊYi›Ô»$²vVoÅòÚhdݬþKÔ±"¹•3"ng¨Ðlµ¨
³º#þòˆ:fØDø;K‹ôKƒ
««6ôhæ¸ç"pÁ|™¢™"g–ÔÔÏÖó} â{s2AǐŒ¸Ã©)µL	•F£<Àk4jyšZ´"©Z'8 …BiI^ÀⲸʝå$@FrSoolâ	2gîÄc¯|Ñþ›ß´"§'JHDô±BvŠÊèd`ÊÂII…:_"=¯Ñd#5û>5Š¯˜Näe•#9 M)m½"àŸÔ[
™yRMù®!3º×kf,kŠ'ڍ•½3«W†65äf_ž™á®q5‡òëòé'%ÝÊó¾ÿ½e3×D¢Cá®ÂKîp"½¸µÈÓ\ÜÐS0I2SzéÈG9ŠÃif…?3ÓŸ™Yˆ"BѲp}Ì&TWؒ¤•ùåe5Dy6€tDŠ¦Ië±Ì^Z¶º¡6¸®>º68§vmÙÒªÚ²ÒH$À•gevEòkóݑžº\zÄß]6X`뭩鯮³Äè^[Ö]r§¿6\\R—˜ØêÌ­+,¬Ë/¨¨øƒÞHÇ "™a½Zv
¯VËÄ$7¥(dB!£hÞÒ§ËíTºH@Oî|·YAo\×5ñç–'ºrqˇ1ƒ%í…èØsGß)ŒÊ{@`§èoé82Åx4%%™aN¹š7§By5¤sã1îìV›Ròk‹¤J[ÜçEEÕ²sýÇRÛâùC—\¼¡eC견›[‡Üþîýt|¨Ï:·åš]?¸n	ŸvÞ%…3ª¯ëÜøsTüfCBǠ߇µÉ–=|²IcÞÃkdg3™h…RG\N£ÓoM-+"bm@µM•3ú›&N"¤Pg¬~éœ_ÜØ°¬™þ²ðgzn*ÊÉ¡cú‰[×_Xpæ%çv1·ŠütjQ£T¾‡§T¥4©È^•`×(qZœ§ÑetÒÀÄvÒ6!,#¯Ñ‹ŽuMÜMÇ@Ð
ÐˤuÒÃZȕª$"ÒDdâ"!É,b¬F1ºŒZÐÓ7±«§ïõŸ)£þ3OÑ1P³Sô%:=²Ä½«ÌWóªT8¦©ÿlŒ»c
99'!ÈÖµ7/ä,¼qÁ'k‡k6ÎiÜ8{ö††¾CÇÿjã†_õôþ¼Óo—L\ÖyI4ú>vyÃMHhý1:\˜¶(ŒgÜÃs\ªYcJ5™³¯æÍ	mÄ=,'èãvÈ"ÙÄå.¢qkN¿U&ű‡Xþ
ڐ—Ó¿Ò]ãÚ~áâ'ê`Ѧe¤1Ԛo5/
¾ù¼¿œÞœÙîiЛfWúQS4sâ!:–:ñ‰±8-TñŽ˜Î¤"m%‡OÌhŽ$‡-)¶ìݼ-ÊÝ_öK1˟㕶,b;«°x6®(/+&S^Z¿íòUWG˂|—jeëÒ¥¡‹:–îšK)¶uv.»´ª¬>Ú<ŽoêWDëªK9_2Í6ZÖEg.Ÿ\ߨên«ŸÙš­ÓšÍËfW-
€Š_h5!刄]ùiiev{Ùu¼Ý`·ûlÑúô¾ëx½Õ•""ì}<ӏÒ$ÇSc"ʲH&1Û\ùn)ÀÄ4TCÄ¿³GIªŽ&'°†Ì&
â·Ú¬ÇâyIOiW/çȪñ•,³VGk«S˜6Ç•¹ÕeY
FC5¥§ÙªŠž(²çävD\µ&³I.7ª­åE嚮ùÏ©ô.§Û"žmö»ó
 p³ÓämjBz"_(eII)JsÊ>Þl…2±§7_"—UGó}·ffiC[SCuX½Pwþ'Û/£¦î֔â™ý½ËWEƒšEý»/ß~(rÙiò&ƒ	Ùp…S¶}¼Â*3©E—¹×L@Hb0UK1ct•Ÿ˜€ßj3s¤[ 7;ôsf†VΪˆ"6'Næ׺g7Ï«¯m¤cgÊê2'í[k‹Ò	™¨ó¾å‹—ž·TÔ•S¬È"?œž¢Õª6ŵ¼Í¦†A½7XaÿŠ.&UåLâ"™RE
Q:㑜޴¶bâ[I"ˆ©Çr~÷…;ƒë‰SÖ]YÓJMs.šçè\RQ¦i᯺¤k{ä¥yóºÄxQ¤'ŽÃOت³h
j£ÑpoÔSÈäïåAî'.Æ@šx돟̙$`q]FWy ¼¬âxNQŠ=Ýíì´Ì¥ãêfyNayÝD<\7»-
ŠV$ùA.ü¨
gêõÉH6ïã"ö̂̂}|¦E¦§%(™æ塄"&õ!êÁV0š•	UÚ,q•HŽ|6ÏI3i±¤EÁöÌôÖº%Ť[9k¦{–Q¯™ÕYY]µ*Úq4Zmµ³[©i^ÍDÕ¦ÊâªÂè}
áΰYªgä×G.šß¶µnâóށ<AxÉÊ1F\OÇ OØ;å…žP tXºÍw•‹·µëc±XŒöŸ)£
ñL~–á€4Ljì°Q•²—W9'5×òÉvãÔôDî×°Å{pw¥tÿ`<‹…jóÆC¦ö?zf¼¯U=Oé™IÝ ÓäI¾XĵBâm¿$"øïžDü;'ôï	Û4³%ÛÂéú½¼Â ËICÚÞ)½Òâé[zèð[mRXŒ.£¤Ï©†Rj,5"U5²›*Zºb^(óçGR'c­Žj*öz‹ùŽ‰ý¤94³;<q"tWWy
³fO¼Es=3DÉêò–Ž°Ne1YRõ
4{§;Bh2¹Iì§q¯ UUí©ÚäØúQ½6Ö:‹š¼9¶ò'	"¿[ÏUL£ŠÆnÑf.všª©	zØ¥33u¯²"}ZØM?3Ýùg}iòñgÖÆƚ
sëk6tt6D»:æÖwQSÙÖå·ÖÔÎùîÂm5,\µlñÚÕ ÿWy'Ä/3¬K¶hô2º——ÉRä"¿Ã~±¤eÉ©•"š•ÔI|Þ,Îå/Žµ¦—R"£=µgîÄÛTÑâóˆ_°ÉSԄBÂééJ—N—©´fîã­VYR'r*§Nô0ŒñD':-¯ŠçýÒÇôtYDō¿[§Z ¨(/Ÿå*)
µVû—7è*çTU‡BµáæjßBjjœ«uårÖL½VŸUSækòvt¥"W»œœ^ŸYSVX/ú¦'":z/¬ð†­ÉµR«ÜËk­V«Ì"ÔTÓu|ª‰H+NX¼´$UÌ/¢ú+mñЖRMå¯c±Ô,%—R¨H
‡cTQ7ñ@ŽCÞ¢rÎ*&Ѻo—‹>UÇN'ãT›èSZKŠL/ÛËë­j½U/ÞeMò¨œLâíV¹"qGj¨®Ì"Ü©fUá'4&vw°ÆãΜEg>›s¹mU¤]ä"T
ôwÊÔ…>YZ?PZRiÍ&•©™KxNmL±&oîy¸ó'%ÇÒªÜóÒÈì3Ÿ‰YÀ åEQRgØhk)º½|ŠZ,ò"°É9ÅçøJ«MZRG]9ÅDz"Yà%«NŸz^ìGA°8;#™3gçštɏ,ûK¸|V)?óASkqr§Êšë¶S¥ø¬#fþßI™?™¨
gÙ-:‹C?ý°…Ó¾r
d>{"þéQ O¤¿W|^ÃQ50ki™CR6×4ÉJâCåüÖ¡Dv"N#ZFÇ1uaWVŽÅÁå¦'çåå^Çç鍠0™õæ½¼žœ+Ôd'H<©ÒB)Ét$"ˆ"¦uã'NIûª×«³¦g:?mˆ&š†þþØOE™é¸f^'.??¿¼¹5ѪŸ˜Mõó[ÿ˜¸³
endstream
endobj
93 0 obj
<<
/Length 6677
/Length1 10200
/Filter /FlateDecode
>>
stream
xœ½z{\\ÕÕö³÷™00˜`œÃa 03܆[	Ã@!BtN#H äj5ÑØPû¦'IlMÚ(ñVõÓÖVÛ¼«&Þ5Å\¼Æª¯ñ¯Ñ˜¤ÚZÃþÞsfHÐú¶~ýãÛç7kö^kïµ×^ëYk&€Ãš9s‹J{ù-¹@×y
­¡þoÖ^Äß
hv¯¯Ñ<©ù ·w_²žOœ' º!€¼³tMïÊ^ÌہøÛzÃëÖÀ'€o{Wl\zµÔß8‹ã}KÂ=ºà™k²@E_ߒ°î3º 3þGNßÊõê
4K® ëW¬î/ý¨ÿ1€Þ	àá•á
kÈg	}1àW…W.^Ÿú% 9G׬^·ž  "ùšµKÖüúϛN†M-…ñŒÁÅ`ô UGXWümà@ÀAmì~Eß÷4ÐWÆ>ó܇Lb‹¸ÓªŽ‰í•C€¸)·ºÐTóW$p*'Ã<¡N8|â+/"Æ^àNsw 4¶RCséÃÐBC#4 %úM¡"T4Á@Õ¦‰ê?×Zç̞Cn1Ûî"…<ðEFutTñ
¢«8u¥ÈVù<¼ða:ЈY˜ƒóF?V`5ÖãldLÕàE	¦#0aN7V`ÖFç°wÿõóOžúþVÿož¹±çR<FòþÅ3›Ì&א'Èäƒ	ϘòÐ)ßyº¿ç¥£œ'ëänæ^ÓTjú5[5{4{4û5ûµD;E}–k÷j™–éõé$§a<û:뷡Պª‰cêÁêAõ ÷ÿ]@_8û]D_Àµß™ß;·­ã}."dzäßìïAN컀v#ŸzÀ"VÕ~7šˆ3ˆ©V*ý˜M´"Çu-¨§8HëÿT¯¨.íýzzÌWP­‰ð#‹õ	Rq ÖW²ÿéXŸC«b}
²1+Ö×¢™±¾™¦c-–!ŒhE'Ú°«áE=Vczp–`-ÖaVcx" Å(z\Œeê…[¬>çtñª6>¦?«¯UÕ£äÛF¬ÁðhÆJ"Ñ‹eX…^u¼
Ý(DõÐVR£åg9ÿۚVc
6ªÒ^ôa=xüüÙõ<:ѧÚóÏ*k×bJÃXóE!xLÇ
u§sZש£%X§úí,A
:ªäŒJ‹èãHü't0°ÓÊèeSÙ©'ÀÞ¸»Æ.þ—wþk®°+ÖߌA\ëÎò'¶M؈K1—ª¾^‰5Z«,ÒÿÐÞÿ,f_G{~öÖQ»#㥗펌Ë7ٝ—oJ;ü'Ý'qÉ¥vGÆÊ5vGƊÕvGÆòUvçòU›×¦¯¿8ŖÑ۟bËXº,Ŗ±¤/Ź¤oËEéiëì—҄4á†Ý:÷õ»ãÜ»w™Ý7í0¸¹ÃàþŃ{çƒ{Ç®R÷Í»ˆ{÷.âÚ¥w_·Kï¾v—Á=¸EëÞ¼Eëþé­û¿¶hÝ?Ù¢u;+m©6[¹ÍZf3ùlÆR[\‰MWlãŠl(´åæ%MÎ3¸"<nS¶˜"#š2³'ø,ÓñÏ>7šÌc\|'Q§79ÖBN2)1UŸžh3;­š"DOMAÍäšÜÿ¤œšì¾&³ÆY"Zc«±Ö˜jâjt5\
jÚ|D¶¶ ¥³^N&-h™[/ûÜ-#ß!—º[丶¡aB~&É>·L¯!è"5WPtÊÖÀü¡'¦ˆ·8÷€È-][®–ÜîIrOËܐ<0I'K•Î5"$´È¥í²S¬wÿ»6<97(ò'ØÕ0Q@T
•Ê––ŽÐðÍþéœ\N•ëZæþÓÃqÊAÚ:ê[dCG‹lh[ §‹õ-ò³-rEÛÙ(Ö茞Sý)…€(
FüÍÀ`€ž!qìâϾAØadß Q¥IHbßÀûf•Z`f_Ã
û''̾FŠJmHa_Ãû;*M…ƒýiHeG:ÒØßàDû
Hg_a2ØWÈÄ$ö²É¾,ö%ðì+d#›}	Q¥9ٗp!‡ý¹p±Óȃ‹Âdä±ÓÈÇdv
Èg§àV©ì$¼ð°S("‡D¼ìŠQÈN¢Eì¤R‡Ù𡔝@™JËácŸ£åì*QÁ>GÊØ	LA9û՘Â>ÇTLaŸ¡Õì8¦©ýZÔ°ã¨Ã4v~Բ㘎:võð³ã`:û
¨gŸ"ˆzö	`£	Aö1f '}Œf•ÎDû-hfcf²ÐŠì#ÌF3ûsTNZهhÇlö:Ðʎa.ÚØèD;;†y˜ÃŽá<ÌeÇp>:Ù1"0ƒ"¹ì}ÌÇyìà|öBbïáÌgïaæ³wq!°÷Ѕùì"±ˆ½‹ÅXÈÞA7.`Ø;X'ÙÛXªÒ^"ÙQôa1{ËÐ͎¢Ýìm,G;ŠXʎb%zÙQåŽeoa5úØ[XƒeìM\"~ö&Öb9{밂½‰õXÉÞÄÅXÅÞÀ%XÅÞÄ¥XÃÞÀ\ÄÞPª2{—©ôr¬c¯cÖ³×q.aÁp){
›U:€
ì5üÙk¸—³×ð•þ6±#؂+Økø)~Ä^ÅV•^…ö*ñcö*"¸'½Šm¸'½'íø	{Wc{?ÃOÙËø¹J¯ÁVö"và*övb½ˆ_ Â^Â/±½ˆ]ØÎ^µ¸š½ˆëp5{Cø9{»q
{×c{7`;"±"ÆMø;"›±‹¯p-;"[p-;ˆ[q;"Û0Äâÿàzv·«ôÜÀà׸'Àop{wâ&v¿Å¯Øóøna£¸·²QÜ­Òßã66Š?àv6Š?â6
w°ýƯÙ~܃߰ý¸w²ý¸¿eûq?~ÇöãÜŞÃ¸›íÇîfÏb~ϞÅCø#{'ÌžÁÃfÏà³§ñ(îaÏ`/îcOcîgOã1•>ŽØSx²§ñ$FØSx
{ØSx±'ñþĞijx˜=çð0{ûñ({Æ^ö8F±=ç±=ŽxŒ=ƒxœ=ŽCx'=†Ã*}O±}xO³Çðžaûð2žeûð
žc{ñ*ö³½8'?³½x
fâ/e{ñ:°Gð²Gð&±Gðß*}‡Ù#8ŠÙ#x/±Gð^bã]¼ÌÆ{x…ý	ïãUöŽá{à5ö>Ä_Ø|"×ÙCø¯³=øo²=øÿÍöà8Þb{ð™J?ÇQ6'x›à¼ËÄI•žÂ{ìœÆûì~üÇØø°ûñ>dàoøˆÝ¿ãcö¾Æ'ì~üŸ°{ñ
Ž³ûpŸ±{1†ÏÙ}`øœÝë?Á|i^ç܎¶9­³Zf6Ïhj6ê§ûëj§ÕL­žRUYQ^æ+-).*ôzÜù"ór]9b¶ÀgeNÊp¦§¥:추d«ÅlJJ4&ÄÇô:­†£'*§BÁ~9-Ð%ÅÑÌËÆÙ'Z‹dX'há}E'76KÖºe$·È)m¡aø«$Yçþî"Ù2ç2ŸdX[|PÖ¸dKœî''w"ÑüŠó¬\'¼9=§L]2u5˜Kæ\3Ã|ln	Š@å4Ëh)ŸöN•à"Q%HN!9s|(Ißgä€íûŽ™³IÄ<lL4ÈH†ñ6eډ*Ȩ''»eê2˨Qµ¡H&)'e',[«ë··P–­ú{úÅ`Ï29-°¤¿ëœSOD]*ð>Ò²øœ' ZÝ"?ÛNˆˆ%ñ'וáø"€HP²Q\3LŒµDíPc°z˜ÂèõÈVÅÞ òé—ýÛºdêAðzääs'¶oûDd«{¼—íEuY5'_&ûÃ2¶ñÞ}'í#f,îr{Ğð̅%¯gœ+Ø×)g´´Íɜ+¨|ºúx%Þ
*Q¢ÇûøˆØ ÈúºdÎ%6(Qÿ¿§oI—'Ò%6x=r\ ´UØ甭ÐÖ lqˉbƒœxÙ{N.L]Æ+ÃHd+/ßÒš(*IRª×ÃG'b°¯«Áë	ö×+1):7ŽÍ=jtüÛ¼<°¸?
¾ðöñ"fÙø¥àAP£.Œ¹²§«_1¹?¬3ØÏG¶-Qº]=š 8ù`ƒòQòAóäÔÀüP°OžÛˆa^æ\ß]+rš[Y‰Ã=õ^OÔd9Í}Î~%)œn"SW@öwª_èTcÀe¸AŠ±bæ+ËIWƒ$	Ѹs.^Ö»¶jE>¢hÔ»ä·YxRðzöy=-¡`ƒS=½L¡siÜ–­jvÊÅéJ&,HΈù¸äõ´´]DR[:B'¢ãΨ[æŠ-íQŒô"®Îh~Ó³¸)6_ÙsÚó©Îç£}™t(sÁÙ(6vE""ß銄GØÀb'7‹'a£1²&ØÅ«U'"GØCۜrãvI6wõ'jË
6;ZääöJ(ù¾p´²Ô‰B•S°œÓö¿‰c9)ë²NÍɈùS¯G6B'"oTjÑ;Qå"ÍUJJó2æ…FÌèVñ­'°Œ¹!™:•¬â$WpÙܘ»œÂ8¸""ÙãJ^ (ù¶mďÅ^ ´‡¢c‹÷À_ä–dÚ¥HöKlóÉÀ¸äìò.QðzR•ßiþ%þ'b?b­ü""5jmî'÷u†FØߪdCUɁ礱urJ/Þ-šùÙáV*>''»#f'?$Êf·¬
"ö9k$Þl'a%^<ídu™‰Ï¥Ð"Å,"™Ø>'e¢ÖÎQ%"ä³P⃑®Ö&+v[ôô}ÿÙdË,ÊÆ/Ñù«¨œpT-±²îjTòÎ)Dg̔ä$¥vËIŸªÄ둝/"® ŒvµÃù>%Ø2ßÕ –É9'=Žv5(%RI"^±9
rÉúw°æõüPˆlsÊ?Þ.õU{=²¿@ðzør™t©ùÒŠy©ÊË)e¯få(ߖŸõâøœH¤¹AMäˆYxÌ)ûÓSc©ýO^oéüÖhÂ~ª¬êlñèɍîqýÑq"Û9q8ã;âæq1dê²(ÐëçÕÜñwÅÔ~KÐ'ýáñ;BW8/S4YÑBZ:뽞aŠúa'\Õ>ì'W͝Úcø«:C÷PB]õÒp¹ª=´‡ü*—*\…©xe hêÝC
ê|ç?0 J5*Cw¨<Ã8 {"FyæèF¹êF~Pth¢ÿøl
ºGQހÊSÛ0‡øãµ~ƒ?Îo¤‰Ôýÿ­ßðò²"à^#I$ÎáèPÙ#d`8ÎïŒÎ@ñG-¼jÞ¹­çÍÝkD"qªT'¤z¥y=ÁÔ>±¥=$òA¾Gö·…6I}'.ÌLm2Q´@)ÿ2Ÿþ\¬ì˒[)†ï{h•¿K'ènpÐ!F˜PãO0éõ‰]||'6á!vqì"?1!.'XfƒÙhÐR=_ZZUU§R‹uŠÅ§''â|bô'CŸg©tXˆG>s'×g=rÛ¤[ÿrÛØ-$p+Ý]tªàäXÆÉSäý3_œAö' ™†a¢è.)v	å	Ž"‰{A0 zqÈz€¤j´×Kšvâ~†Rƒu>‹¯¨ÊÔº'bA´èô嵤ÒG"'YK*7¥®¡ÚÆìM)‹@¯éAðpûm	))άÌÌ$§%i·dIåœ7HœuŠ·ÅŠ)©E>‹z¨äZâ+Í$¶"$¢O"zÁ&ԒÊZZ^–+fëôyÝ|Ø׺´¸hF;7'XƲçõÖV;K<ÞÍ '^-ÕK«Ãmy¶ÖŸ"«kËyoiùÔ¤°òW \všRz4ús¬ÉÉö̬Ì%}FVVƯ¤¬,;'ì7HIiùù¹È½A'b¢¾Ô"߸™ê׸É%ÅDµU§Z,f'¼ÊLâ+­P
ÖWújɸ鵄$N—–—Ô6ûWÕ—Vë·h|E%¾Ro¦`â*«Ü9b‰nsò:z°rž§¨Õ™¸`º¿ojåÂJsAms¡7¿š"äÛÃó}ÃGÒQèI~"Û)Z±j­ñ:u¾º:‹uJ'[‰Sž ‰óqôà͵cïL½ž8vÿñÉîÛn££csH<ŠØiz3=§-‹Ù¬ç4šD}Jâ)%ú4ߍVôøv‡¾ˆÙ:[ŠÝWZQéˆ:¡¼¬–+V
¥ý<±­ºsQkwÝlËöIׯ
ÿ²½áZzdyov•ÿÒËÖlkkò\¼vþí«ßµTy_Co¡£H€¿QoÝ)é­ËNÉÀÅ6/)&v[Š^'
¡ÔΕ7±øJk	­\vAóÐØ1â˜Õ£)YØvކÀœ|:¸èÀïϦ£Yc#½½üX®¸Dy[EËé(â¯QíNIÁµÕ@Îmõl'M°ˆ–ÝA<c/]C>¡s·qìQÞnÑ …¦9ì"8«†Cbc¥²Î÷&é3\³q£ò²"ÂÍNÓ£ôL˜¤œÍ²C2$Ã9Á±ã`:çA.EÒ8'È–‹nœ=÷ÆþÕ7µµÝp^ÅüŠÒÐÔE}½‹è'®;—¯ýµ´ðŽ•ýváØÏ:W•®^°|0}÷ÌýQ}'áO2€ãâôÖx«†$(Qâ˜RRìJö9‰ˆÈùˆæÊ»7¯Øù‡ë~õMwýò(ùtÌHNŸ)£Ž3ÑQPä°Ó4žZ! u~!Áf+t8
»%‡Ùᘌ8[Òä&)ɞ•™é"sH'yB
!U…d•
"K,}LDgwˆ¹yʹs•cWVTžË™dý8´*¦±vw¥BŒÉ[µ‰®9ÞÖ§tT—?¹<rü¦"¾ÅŽYnÁYaJÌ£Vß܆ëšü	…9¼†)Ì³Ùž%ðŽYMc‡µæÒÌü‡Í—oA;MS¨éãØ×hµ‰úäÄë¤d;ÕIÔü}ØO®ð•:ô¹°¯³ó"ÈUô.ßS¸ÕÒZ6­¬.¿$nkÁ3—ø…lž<9ûŽÔŽís"":žáꯪîQ°'ÏNS'ŽBñiž?…Ú4v½}HÒÛ-Y¦¬!Éd¶B¢e>¥ö‹X.žƒŠ¯Ôaáb~*/Ëu"$BÅ*H®)ÝÓ¦vׄêޛîqV¦XýeÚêR:z¦lViní¦ùço˜:ƒÐ±ŠóZ2òĦ–6îBåÝ=;M5Ô
;&¡ÔŸ–¯×84ݒáG'~HJ²Ÿì9¯L¬‰v› Áh9ȋš¨÷©…'$mºlìN:¥"Û?˜¾¾ó
&ï[nzžLË/® Ö[w•µˆ.ǬÙ-bYӳߩ«*•[¹;ûé8PèOµØLÉƔ"ä!)ŤÕ5IZp†!‰#1ƒT£à³¨ŽR/"hœ&ŸM´ˆ±ÜW^vqŠ¿¨ºÊ*f𩽽ƒ³fÑߤ¥ZºY™ž•c½d÷JßL52…TT±îE…?#)ɚž`'2®t×uRºMkâÜpO€y]ì+æŽh‰ô•û,j^çæ9TÇL#âÄ4·_:¢)Ÿ"F&/ïþÑ:r"&Ïå/¥éí…þpy '½lª·¥Ò_[J­…¹3ÆrÏ_Y-ŸœeóV…r6Ìoð}3ý'Æyuv 	 ™tv8ý‰ñ)6˜8Ӑęm*˜T#Çï[»Ãn³ˆ–²h%·ˆß!±ÕëؽƒÆ×ô¢ÁAòd¾+Ýæ¹dl/É)ªÊìlû"Zהwì‡é(8èaóÇkm:%»$Šh,"ˆå>EåáÁÁÁAÚºùLÕ"½À
q@]i…è·&ùã2Œ»¤§õÛ'þ|T-êƼJÕc–ƒƒö†úœšÔ]Ž¶n~úÌWP™ébM^)a
jÎY/±)*ëJŠ}Qcû£^Ê¢V¤)^2¤Øl&‡Æo4vÏeÕGjaJ""ˆhñÙj	Y[ؐ'jäËJ*´7x¥ý|jͲ¥7¹Çþ@œ3«\©¹©_RÝ,¡"ÙiZG­0Á©ÞÉ×I;Ò®;—LßwL€‡¯ó²Úéۃ—µNۘß\^>³iJY3µÎÚœqŬ)Wt6Îûbv{[ÛÌÎÔd'µÂŠ¿ÕhK4i¸]'FcÒA·ëì}©E±P©×y®˜=~<_-!Uö'd·8)orâàfšVJ­I	ìåιêšÜ p°ÓäԊ\øüiŽÔT=o4¦ëSқ¤;§Ñè¡oúö--þ–³Å"ú"-ÅîȤ¶XšTÆΜWHËË*ˆ6¼Úve\QÁÓª›æW—ô·/ØfL^˜S7‰¿°¿~µú›Sù,·--Ñ,L¯ðÌñÍî°ÍMãm½-§¡º}¶i;M¦ÓG'Ž"Z'áZ)ɞ?$%ØÒÓœ‡}Hr˜+_jÑxD'}6ѦÞÅт–›WH¦¥ŠT¹à­ÙbË6Újœy5I&}]]"êV¾'ðI‰ýñ	éö´i…_¬ìmQþ˄òêÿ$ÝÏÅÛô	&åg4Ø»ÃWQ™ìãDÎ÷e²Ž£¦Äî«l:|
!Óì†*žÎ|­äžÒªC2x¿Ù˜"—4$ÅeÀb£VU/f~I±Ë—ìãôITÌ."ê½ÀùH
Ýð³éùs'ù.£hwYžÚy-Y3–(6·–뼕Tÿð÷m
endstream
endobj
94 0 obj
<<
/Length 5289
/Length1 8424
/Filter /FlateDecode
>>
stream
xœµX|SåÙÿ¿'Í¥mÚ¦i"¦=¥œCH[IÒ[€(mh'
D -r%VJåR·ic`Pç
7¯Û·±}›¾•â
†âPAÀ)^pˆŠCCÇ´Ï÷;')·¹Íoû¾÷üΓç}žç}Þçž6`²Ð
º&M.¯ºÜøƒ[¢Sƒ"óÖ^éÒfúýsĺØWÂ<€ýÀÌ9W/•Ò¿6qÀ0`]Þ5wÁœÌßìA í±¹±%]0Að5óÜù×^^¶i׍€¥0˜:ÚcmǑw6ÀðŽŽö˜q•~/ÀÆܱ`é5ùƒ…G].ÀÚæ/šÒåy¢ž\»¦‹}–¾`&ÒÂ؂vçÓ£ŸR®Øë]‹–,¥ß 
`¥*¿kq{×/^»áÀä"200!YPã  #¦A¯í
1`®´Ç ƒ =¥êû–ÅaOßçئ;Õwºï©—îS¼už"¢ieÀ=^ùø¬¬Ú/'®ûTeì>¸~†öyìTEßé¾Í).ÝZHM¤!©]§6#M,°¨AB&#†yX"«ˆ4Je'2K‰èãsMÇù+EÈdwB!.DèÂê'ƳËPņBº^!UHIØ~vM˜4q»®Jú½–ù%à•'"íš-ꩆïøtâ™ÿôaÿä¹ý'g­ölò"áö3Ïkº!'º3·k¶ÿWKðà^ÁƒQÿ¹¦ÿЎŸ ñß:ççŸ
ìCÑ9xndÁ£½•Š2;j_#¦«U'
àFœLâìKâÌx#‰ë0W'ñ£)‰ëQ†AI܀AÆ`1æ!†ù˜€V4a1Á‹qXªÑæa¦¢‹±D뚅Zǔ¡Ð€«´ÎiÓ¨ÚsVŸ¤i"':¥ótNÐt-ÂR\‹.´k܈a.æa!æjû…˜ƒ2ŒüŽG¢
¨Ä°ó¨ÿèl‹Ð…k5î\t`)$üJ›	ZÑ¡Ùõ÷–ªg£Kƒ1,MÆ¥Æ`¾vÓY­K´];–h1¼íhC l‡9	+…-ȸ '0£>1Aυ4'Ný;ù—nmßæÿ[ÿrÍB³'øDDÁl
o½@®"0ã1cDµ¶±ïÛúrÌÿ³Ýßq±yt2ùéƒýö¼Â7ß²ç^ƒ]¼þ†üÝoØó
¯þž=¯pA—=¯pþ"{^áíâoZ\°ôª\[áÜÎ\[áåórm…í¹b{Dz+ò—دäË×ò埬1¸X"ê^³Êâ~ð."ûÞ»Lî{î2¹ï¾Ëä¾kU•û¡U̽fsß¿Êè^½Êè¾o•É}ë2½û¦ez÷–éÝ?\¦wß²Lï«mŽá6Û0›u¨-Ëg3WÙR+m†
›®Ü†2[qIfiIÖw¦Ç5ș9ؙU40S˜uäó£æ,K¶95-Ýl0šÌº½L0‹l@†ÃXa³äeXSr3<µCjKk‹kýת•j‹jÅZG­­ÖZ›U›Zk¨ÕÕ¢¶É×ʸ5ŒpkÏaa"'7pŸ;Ü«"Zx•;ÌS›fDz»Cá>7Vô2´ò"½Z¹50}F¤—å«ìeâF0Ž.»]q»ð¶ðäï ð*¹s€'0¯j梳Áý¯VOiqˆ	Ÿ'
žË`"yv¸%Òó?¨œås¯Oþ»zRUGšZÂÜÔ榦¼ÀÙæÛZÂ|xÓnv6ô0!КðSû{©f|e"˜`¤>¤"•¾AÒèk¤#¾†fúÌDý
YÈ¢¿Á¢ÁlXè4¬È¦Óȁ•N#9t6äÒiØa£Óȃ¾'vú+ò'G_¡ùôD
¢€NaD:…"ÒIÄ@:		éKȐèK'L_Â	™N`0їpa0@1\t%,E1}‹PB_`Jé8ܸˆ¾€Cè8¼pÓq"i°:Ž
"Ñ_P‰r:†*"ÓQøPAG1UtÃࣣŽatÕFŸ£Ãé(F š>ÇHÔÐç…tµI‡1£èê0Š£µt~Œ¦Ãƒz:ŒÔÓgÀO‡Äú!Œ¡ChDÂÅÒ!ŒE€aéÆãb:"0ÆÒ§¸ãè &`<ÄD"é &á:ˆ&
6cD&џ0"è ú­JŸ`
šé¦¢…`ZècDÐJ `
}Œé˜B0SécÌD">Â¥˜Fá2L§1K£D1">DLƒ³q)}ˆ9Þ¦áíˆÒ¸1ڏ¹ށíÃ<̦}èD;íÃh£}˜Ëi`.ýQý®¥÷±Hƒ]è¤÷q¥ã
ڋ%¸'ÞÇŖ½¸
i/®FíÅ÷°ˆÞÅ5è¢÷p-®¤wqÓ{¸WÑ;¸Ké|_ÃoÄÕô6nÂ÷ètãڃ›q-½à:ڃ[p=íÁ5¸7Ðü7Ò,ÇMôVhðVtӛˆãfz+q½‰Û4x;~HÀXFoàÇø½;±œÞÀ]XA»q7n¥]¸qڍ{§]X…•´÷ávڅոƒvâ~ÜA»°?¦xwÒNüwÓëø©Ä=ô:½ô:Æ*z`íÀ£XM;ðî§íøÖÐkø¹ÿÐkø~J¯á—x^ÅZ
þ
Ñ«ø5¦Wñßx"^Åoð(½'ßâ1چÇñ3zOàç´
\ƒ=ømÃ:ü'~õXKÛð$ÖÒV<…_ÑËx¿¦­Ø€ßÐVôjp#~K/á<N[ñ,ž —ð8mÅóè¡ñÖы؄õô"6c=mÁïð½ˆ-xš¶àEl -xIƒ[ÑK[ð26ÒfüÏÒfló´	¯à9ڄWñ<mÂkx6a;6Ñ&ìÀfz¯ãw´	;±…žÇ.l¡°/Òóx[é9ü/Óóx/Ósx¿§ç±Ûè9¼Wé9¼ƒWéY¼‹×h#ÞÃvz{±ƒ6â}ì gðG줍؇]´`7mÄ~ì¦^|ˆ7¨áMڀñmÀ
~'=´ÂÛ´ñ.mÀ§x—žÆ!¼GOã3쥧ðg¼OOá0Þ§'qûh=>Çô$Žb?­Ç1ì§'ñ|HëqÓ:|´'p€zð%>¡u8‰?QNá ­ÃW8D=ø«Oã3êÁßðgz_ã0q|ƒ#ôúð9=ÂQzzõïx!_XH…Y¨õ§g&CZZº>ý:†T:æÏHOÍ`V³Åd1›ôÊwTUÕÔÔk0Û:"Û§ÊŠ‹X¶l"óŒ%ÙÕyÙL.òû\lï%}Ï?6àÑ÷ë{"֔1äx_áñ/Ø'ßüå8îØ~a'Ò0hƒŽ¥ê
k}/{Z¯OeŽT#êë­#ÊkÜÙVŒ¨¬9%cu«ö±q'+…ÐòìñJCQ¨q5
ì¦þŸ&T	;!£ÊŸŸš"#šrsÍb–y'åXT$B|Xõîløå¾zMs¶/[ó€U1[n&Ëb™Ì(å:¡žÕ	Æ;Œ%uŒEÇ̪*k5+¿!‡ù³û¦f¸']RZÓ0ä⪑¡Ì©×
;‡Mê›,çåæÑ-"FKÞэ%U¡–st¡úÚH'"‡"wPŸ?_Lí(Í̔Œ)vØ¥»{Œw+HA½Ž¤mÉ;ÊËUíyÆ2æd°å±¼"AµÖ9¨¸¤xXµ1×cƖ±'2aØÐ:ÆÖÜ°\¸"ͺ¤zNÑÈÑS§ø'7¶4^5xØ¥lZ[MS©5Lî_,¼³¸ÝVŒ**•\•ãjFFk×,6å×MuÖȇ
(5µ<tBȬpa(.ö»
²K¾ÕJ¥ Àn/¾_±Û½È°ey­ÞՊÕé>–~oàsÔg[G"'bŸHª#á•-אÅ¶\»ÍY\¢¹4l¨šg՟bç 5ø9™'Muq¸J7°ð"EFÀŒ4Å ¯˜æ\z(PëÐÊÊÓÅë+Üc†VT
np8òÓJë¸Ñ–ŽT˧ëujj|8U0¥f;MÅÎY¦IM}ûu™C.\5°@l–¥þ€V0³°:'õ´ÞfÈbP¿£¾¾²"ÇYíÓ9s|§›r_d¾"t´}3T0€¡@ý-K;•¶žÙÔõ•>gŽo‰r_DØÐy«úw†?Ïl+°•Ú.ÊÒ[ïSôG:­lø|-hõª
5ëÃ}jŒ:gÎðd=f²³»Lf4d1gŽÏ˜WÇX·¯>mRtt0­1rqª4 ´9/#ÛTk*­5£mÖLŸ² bJ&Ö¡ÞØÈQ…å}³)e±°¢Ä6lpßßØW¶C¶Vq5œ"…2_ÂvÁ"XQ€B¦Ñ–k³e9€Œ³&;ú=ßÎs»µn\Æ¥1µ¤È­ægU*šr"‹Á1pTßV6¡<g@Q•¯bÜaÁ0Mç•tB(¬ÈÄäùÍFëjÅhGÁê³e•¼R-š2¦–½.Q%ý'aá˖"oš026"Ð}ńŠP,Û8Ú?jšG°.m¿ìÞɳÊý3úžk-X8¸62é0ÔÐ)6Fx¸ýö4SzF†i•'a×åÂfË]­hž×kNgûÉÏʊŸÑ©3Ør}UÕFC¢"Õb©gŸM˜6:­ÄQ˜U$•ÍþÆÌF±]0ûþXi–cS»³F±ª`÷huBÔÑ	Á+qδYôVý}ŠÕžž•Ÿ…úúd¤++ª
Z7T×±zæÓ9«K7¯Îñý,Ãå;ª` ¹<2¿%W˜1{x"1­.²£¦ Hn(j¹ÿ›Ó3…NuNysû§Í˜®LiÜÒ4iÂ%áñãÆ^Ü
ÆøëëF׎9¢F
¤¯ª²¢¼Ìëq¹¨´¤Ø5Ø9H–
(òyv[nŽ5ے•™aNOK5
úÀàaîDB<?åfgÐi'¸yâ±	åVQvfK¾rś"âz7GN˜ç6Ezà¯Q¸Á}¡ÈD®sYŽËÖ	¢â).žârŽµñҖˆì´ìÏðÅë၈,‹\pqÁ5Žë\\ç"Ú¸¥)"«2Ž£)¢¾½ôQ,rÔȊÈÑáEý[Eù6#7´ù3'²¸¥ÇœräöÀü‡M;VŽZ^êæ'ËÂQ«iC9g¹Ç9ËáÌ6Ãzþê±ý5߃P[§3Ô6çÚ;£gƒz,RYŠKñ–H¶O"eÍê0ßÖéIO8íiŠ×€ž´ô€3®¸ÙÙÕÃÌuLCshdS†×íª½!õíäþ•Q.¸œAY–½žs–ÓK›o;—nu÷c9	,a7¸1a"4ûc+¥Ïæøm½̎ºÍmζØÌ×ů§:W¨£•†›¦G¸ÎRßh‡¤æ;¨5{R¨CŠ;ƒ*¯#Êu.gPÍúyô¶Žö¨Z',êz=<5Y.o¹5YâÙnžáòŒëˆºxÈ1OR·ñør‰?Ò9—+«PQ‡×#ÅCÎPG4èõ":Ԝ"ŸÉ›VŽãÚ´ìøWÆ$Þ=»3Q|±Ûú@Ž[¸ù¤,ʲ,«éÑ&CÙíTMn†:¥øÊvÍÕÛ4×dY"BAõUJ!Ž)ܘ	u8Cg/"âΘÄu®ÏÊ2Ïw«ãñjb¬­ÁëI˜ÌóÝgíW›Bt3.¸Üߪ} UˁâþXPI''ÓÕc*'T9'wKâF×r}™SŠ«.žë¶È/É^Ïf¯'Ü	EÍ{."gÛ¸-Æ­ZïyEÚɟɊ·Q¼žpәCÌn‰Äˏˆ‰†';Ã͉éèÑÖDgêB–•¤¼zçèqGç¬E••e±ÑٍǝRc<õR÷l§dqÆ{ÌæxW(*iS'Åz陕"o¼Má–h©Ö²Z›-ažÓ<CMe£ÔKL–z§\#ÊÙgdšþ;ٓÜà­'ã–Ã^7"²(5ª³¨—ŽÕˆÜR£¶´Ä1%ÒkÁ­¾5ã˜Ⴈv•Nq…æMN†K"û‹K'ÍIªâõȲÚo+{ý˜íõȼ»9'ØK˜-®ƒ¿Ü­p!ªr6÷slSTNw?çÌñ¨Sözêo[ÿ´þÏ­ýx¶Ó*(×2 Íæ6¾¹5ÒK_ÕpSM²4r($1AÔ©XšÛi'jyž[;¨Æ"—ºã§´ËÉ-n®D6‹µŠdÉæ°2¯‡u«&¸,»œ¯0uÐ"×ÂY-gv•Žδù¯Ë«á,çL)I¡x4Yk纕ü¶hëøvßxŠËâäæ"bB>ÛêT=Ü®¿äXw5ª}'Ê	‰ñ
ÏTg7Ï<¬¯‡‹ˆÄY4ÄѬ!RHêP"Í¥hPŠx.¹—öGƒêˆT›HRmN¹"&
ý'Zóz¾k‰w¯ùÍ·)#½î"{=Ò0΢Z¿´F'Qª"=¥Þ5Nuå|þ™(öËÄãã'Z#Ç-òïDî/p$[ûï¢n=owÎ}¯æÌðhðFw¿þÄþb·xîvììqýlpÁ•­–^§¤õŽ?šT{£9Âý±þ›["߯S5YfáÖ¯§G@C"­hîñ³"§G6ZiEkdÀ"@´AéÌV4G6J€_£
*U%ªIݨšZ"ë"&/nôÝ7E#hû9½ÍÔOc˜Ó+$h–ÄEÅÚE~˜Ó›'àøû¥S0§×" uk4mõ@
ˆ?Mï7ùSýf!C¿ý®ÓûMÏ0 •a½™e0±§[´hä^ÖݓêÝHeþ"…+¦œ½zÊôÈz32˜¨AEQÔåõ"ÎpsÄ)…¤6îoŠÜ tÄ£ŠZ4Ý\4q¦&h†:þ¹TðJrìsÅ­ÃO¼ÀÿìF~‡
endstream
endobj
xref
0 95
0000000000 65535 f
0000000015 00000 n
0000000382 00000 n
0000000439 00000 n
0000000533 00000 n
0000000583 00000 n
0000000152 00000 n
0000000651 00000 n
0000001059 00000 n
0000001132 00000 n
0000001747 00000 n
0000001827 00000 n
0000003031 00000 n
0000004236 00000 n
0000005460 00000 n
0000005515 00000 n
0000013859 00000 n
0000014275 00000 n
0000014450 00000 n
0000014529 00000 n
0000014599 00000 n
0000014678 00000 n
0000014759 00000 n
0000014838 00000 n
0000014917 00000 n
0000014996 00000 n
0000015077 00000 n
0000015156 00000 n
0000015235 00000 n
0000015327 00000 n
0000015406 00000 n
0000015485 00000 n
0000015556 00000 n
0000015635 00000 n
0000015716 00000 n
0000015795 00000 n
0000015874 00000 n
0000015953 00000 n
0000016034 00000 n
0000016113 00000 n
0000016192 00000 n
0000016285 00000 n
0000016364 00000 n
0000016443 00000 n
0000016514 00000 n
0000016593 00000 n
0000016674 00000 n
0000016753 00000 n
0000016832 00000 n
0000016911 00000 n
0000016992 00000 n
0000017071 00000 n
0000017150 00000 n
0000017243 00000 n
0000017322 00000 n
0000017401 00000 n
0000017482 00000 n
0000017561 00000 n
0000017640 00000 n
0000017719 00000 n
0000017790 00000 n
0000017869 00000 n
0000017950 00000 n
0000018029 00000 n
0000018108 00000 n
0000018201 00000 n
0000018280 00000 n
0000018320 00000 n
0000018362 00000 n
0000018443 00000 n
0000018528 00000 n
0000018575 00000 n
0000018608 00000 n
0000018668 00000 n
0000018701 00000 n
0000018761 00000 n
0000018794 00000 n
0000018854 00000 n
0000019007 00000 n
0000019157 00000 n
0000019309 00000 n
0000019662 00000 n
0000020091 00000 n
0000020398 00000 n
0000020799 00000 n
0000021030 00000 n
0000021387 00000 n
0000021592 00000 n
0000021667 00000 n
0000021870 00000 n
0000021945 00000 n
0000022153 00000 n
0000022228 00000 n
0000030090 00000 n
0000036858 00000 n
trailer
<<
/Root 1 0 R
/Info 6 0 R
/ID [<536F99B0ACC2DF8BF5CE7C5BB260C26B> <536F99B0ACC2DF8BF5CE7C5BB260C26B>]
/Size 95
>>
startxref
42237
%%EOF

